Does GNN Pretraining Help Molecular Representation?

Extracting informative representations of molecules using Graph neural networks (GNNs) is crucial in AI-driven drug discovery. Recently, the graph research community has been trying to replicate the success of self-supervised pretraining in natural language processing, with several successes claimed. However, we find the benefit brought by self-supervised pretraining on small molecular data can be negligible in many cases. We conduct thorough ablation studies on the key components of GNN pretraining, including pretraining objectives, data splitting methods, input features, pretraining dataset scales, and GNN architectures, to see how they affect the accuracy of the downstream tasks. Our first important finding is, self-supervised graph pretraining do not always have statistically significant advantages over non-pretraining methods in many settings. Secondly, although noticeable improvement can be observed with additional supervised pretraining, the improvement may diminish with richer features or more balanced data splits. Thirdly, hyper-parameters could have larger impacts on accuracy of downstream tasks than the choice of pretraining tasks, especially when the scales of downstream tasks are small. Finally, we provide our conjectures where the complexity of some pretraining methods on small molecules might be insufficient, followed by empirical evidences on different pretraining datasets.

==> [NeurIPS2022-axive]Does GNN Pretraining Help Molecular Representation_/abstract.tex <==
\begin{abstract}
%\vspace{-.5em}
Extracting informative representations of molecules using Graph neural networks (GNNs) is crucial in AI-driven drug discovery. Recently, the graph research community has been trying to replicate the success of self-supervised pretraining in natural language processing, with several successes claimed. However, we find the benefit brought by self-supervised pretraining on small molecular data can be negligible in many cases. We conduct thorough ablation studies on the key components of GNN pretraining, including pretraining objectives, data splitting methods, input features, pretraining dataset scales, and GNN architectures, to see how they affect the accuracy of the downstream tasks. Our first important finding is, self-supervised graph pretraining do not always have statistically significant advantages over non-pretraining methods in many settings. Secondly, although noticeable improvement can be observed with additional supervised pretraining, the improvement may diminish with richer features or more balanced data splits. Thirdly, hyper-parameters could have larger impacts on accuracy of downstream tasks than the choice of pretraining tasks, especially when the scales of downstream tasks are small. Finally, we provide our conjectures where the complexity of some pretraining methods on small molecules might be insufficient, followed by empirical evidences on different pretraining datasets.

%\vspace{-1em}
% Therefore, our overall sentiment is different from the previous works that are cheerful on pretraining in thie field, as we do not see clear and unconditional improvements by GNN pretraining yet. 
%All in all, we do not observe clear and unconditional improvements on molecular presentation by GNN pretraining yet,
%thus finally we also provide our empirical investigation on the reasons behind it.

% indicating a lot more efforts are needed in this field to make pretraining a great success.
% Therefore, all these observations motivate us to rethink the effectiveness of graph-pretraining on molecule applications and investigate the underlying reasons.
%} 
 
 
% \adamsyuwei{
% Graph neural networks (GNNs) have proven to be useful modeling tools for molecular data. Recently, 
% people have been trying to replicate the success of pretraining techniques in natural language processing (NLP) to this domain 
% with several success claimed. However, in this paper, our conclusion surprisingly contradicts to those works, as we 
% find the benefit, if any, brought by pretraining a GNN is negligible. We conduct thorough ablation studies on the key components 
% of graph pretraining on molecular data, which include the network architectures, pretraining objective functions, 
% data splitting methods, types of additional features and pretraining dataset sizes. 
% We start with a baseline setting, followed by extensive control experiments on those factors.
% Our finding is, under every single setting, we rarely see the downstream tasks benefit from pretraining. 
% What’s more, the very best pretraining model underperforms the non-pretrained model.
% Further investigation shows that xxxx.
% Our contradictory finding indicates self-supervised pretraining on graph neural network for molecular data has not reached the level of success
% as NLP yet. Hence, a lot more studies are needed before pretraining can take off in this area.
% }

%Graph pretraining is to learn useful representations of graph format data by pretraining on a large amount of data. Those useful representations are applied to benefit downstream tasks. Current graph pretraining has a few categories: masking pretraing, with the goal to benefit downstream tasks. % \mask
\end{abstract}

==> [NeurIPS2022-axive]Does GNN Pretraining Help Molecular Representation_/experiment.tex <==
\section{Experiment framework}
\label{sec:exp_framework}
%\vspace{-3mm}
%To design our experimental framework 
%To understand more about the 
To investigate pretraining on graphs for molecule representations, we first revisit the typical pretraining-finetuning pipeline used in the literature. \Figref{fig:pipeline} shows the overall procedure of deployment, with several design choices presented at each stage of the pipeline. Since different choices at each stage can lead to different performances on the downstream tasks, 
we investigate them one at a time while keeping others the unchanged. %
The design principle of our experiment framework is to analyze the effect of \emph{every} stage in the pipeline as comprehensive as possible, while also keeping it tractable to avoid exponentially many experiments. %Below we describe these stages and the corresponding design choices we considered in the experiments. 
%\vspace{-3mm}
\subsection{Design choices}
\label{sec:design_choice}
%\vspace{-4mm}
We consider the design choices for the four pretraining objectives.
%\vspace{-1mm}
\paragraph{Pretraining objective} In \Secref{sec:gnn_pretrain} we have provided a brief literature review over the pretraining methods for molecule representation. Here we categorize those pretraining by different principles, and present one well-recognized representative of each category. The representatives are selected because they have more desired properties, such as better performance, compared with their counterparts. 
\begin{itemize}[noitemsep,topsep=3pt,parsep=3pt,partopsep=5pt, leftmargin=*]
	\item \textbf{Masking.} We leverage the node prediction objective, which randomly masks 15\% of the nodes' feature and then ask GNN to make prediction on the node attributes of the masked ones. This strategy %is %from~\citet{hu2019strategies} and 
	resembles the BERT pretraining~\citep{devlin2018bert} in natural language processing.
	\item \textbf{Structured.} Unlike text data where the topology is a sequence, the graph has rich structure information. Following~\citet{hu2019strategies}, we use context prediction objective, which masks out the context from $k_1$-hops to $k_2$-hops and leverages  adversarial training to predict the true context embeddings from the random context embeddings. 
	\item \textbf{Graph-level self-supervised.} Following \citep{rong2020self}, GNN is asked to predict whether a motif is contained in a molecule. The motif can be extracted from the molecule with RDKit~\citep{landrum2016rdkit}. %We denote it as \textbf{Motif Prediction}, and use the same set 
The motifs are 85 motifs~\footnote{\url{http://rdkit.org/docs/source/rdkit.Chem.Fragments.html}} %as~\citep{rong2020self}
	for multi-label classification. 
	\item \textbf{Contrastive.}  We generate two views of the same graph by corrupting the input node features with Gaussian noise. %to generate different views of the same graph, %and leverage the locally normalized probability to
	We leverage the contrastive learning loss proposed in ~\citep{you2020graph}: we maximize the consistency between positive pairs (from same graphs) and minimize that between negative pairs (from different graphs). In this paper, we restrict ourselves to this specific contrastive training method, however, various contrastive learning methods can be further explored. 
	\item \textbf{Graph-level supervised.} Finally when applicable, we use the ChEMBL dataset with graph-level labels for graph-level supervised pretraining as ~\citet{hu2019strategies}. 
\end{itemize}

The above are the design choices for pretraining objectives. %In addition to these stages, we believe the factors in downstream applications can potentially affect the effectiveness of pretraining as well. 
Next, we consider other factors that influence graph-pretraining performance. %the configurations for the finetuning stages in the downstream tasks. 
%\vspace{-4mm}
%\paragraph{Learning hyperparameters for downstream tasks} We find that the models initialized from pretrained checkpoints and those from scratch may favor different hyperparameter configurations like learning rates. So to make a fair comparison, we would tune the learning rate separately for each setting, instead of using the same configuration for all the settings. This is critical for the fair comparison of performance on downstream tasks. 
%\vspace{-4mm}
\paragraph{Graph Features} Each molecule is represented by a graph with atoms as nodes and bonds as edges. In this paper we mainly consider the graph representations without the 3D information. %Generally speaking, in each of such a graph, each node (atom) or edge (bond) is associated with a binary feature vector. The features are constructed based on domain knowledge, and 
%The features prepared for graph neural networks are 
For each molecule graph, chemical properties of nodes and edges are extracted to serve as node and edge features for the graph neural networks. Depending on how rich the features are, we categorize the design choices into two categories:
\begin{itemize}[noitemsep,topsep=1pt,parsep=1pt,partopsep=0pt, leftmargin=*]
	\item \textbf{Basic features.} The basic set of features are the ones used in \citet{hu2019strategies}. Specifically, the node features contain the atom type and the derived features, such as formal charge list, chirality list, etc. The edge features contain the bond types and the bond directions. These features are categorical, and thus will be encoded in a one-hot vector individually and then concatenated together to form the feature vector for node/edge representation. 
	\item \textbf{Rich features.} The rich feature set is a superset of the basic features. In addition to the basic ones mentioned above, it comes with the additional node features such as hydrogen acceptor match, acidic match and bond features such as ring information. This set of features are used in ~\citet{rong2020self}. Additionally and importantly, we follow their setting to incorporate additional 2d normalized rdNormalizedDescriptors features~\footnote{ \url{https://github.com/bp-kelley/descriptastorus} for the feature descriptor.}, which is used in the downstream tasks only and not in pretraining.
\end{itemize}
Please refer to the original papers for the full set of basic~\citep{hu2019strategies} and rich~\citep{rong2020self} features, respectively.

\begin{table*}[t]
\small
%\vspace{-3mm}
\centering
\caption{Self-supervised + \textbf{Basic feature} + Balanced Scaffold. No pretrain has an average AUC of 76.7\% over all 5 datasets. \label{tab:Balanced scaffold + basic feature + unsupervised}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
%\hline
\Xhline{2\arrayrulewidth}
Methods                   & \textbf{BBBP}                           & \textbf{BACE}                           & \textbf{TOX21}                          & \textbf{TOXCAST}                        & \textbf{SIDER}        &    \textbf{AVE GAIN}                    \\ 
%\hline
\Xhline{2\arrayrulewidth}
\nopretrain              & 91.46($\pm$ 0.85) &  84.29($\pm$ 3.80) &  78.35($\pm$ 0.95)  & 68.31($\pm$ 1.61) & 61.15($\pm$ 2.46)  &  0($\pm$1.934)\\
\masktask                & 91.23($\pm$ 1.51) & 84.97($\pm$ 1.55) & 77.77($\pm$ 1.23) & 68.98($\pm$ 1.11) & 61.20($\pm$ 0.41)  &   0.118($\pm$1.162)\\
\contexttask             & 92.13($\pm$ 1.04) & 84.83($\pm$ 3.19) & 78.79($\pm$ 2.52) & 68.29($\pm$ 1.23) & 62.32($\pm$ 2.99) &   0.560($\pm$2.194)\\
%\supervisedtask              & 90.70($\pm$ 0.74)  & 84.22($\pm$ 2.69) & 80.45($\pm$ 1.47) & 69.47($\pm$ 1.06) & 63.38($\pm$ 1.44) \\
%\supervisedmasktask     & 91.10($\pm$ 2.88)  & 85.54($\pm$ 4.57) & 81.49($\pm$ 1.52) & 70.77($\pm$ 1.00)  & 62.81($\pm$ 2.61) \\
%\supervisedcontexttask & 91.54($\pm$ 3.52) & 85.71($\pm$ 2.92) & 81.23($\pm$ 1.94) & 71.36($\pm$ 1.05) & 62.75($\pm$ 2.27) \\ 
%\hline
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\end{table*}


\begin{table*}[t]
% \small
%\vspace{-4mm}
\centering
\caption{Supervised + %Self-supervised +
\textbf{Basic feature} + Balanced Scaffold. No pretrain has an average AUC of 76.7\%. \label{tab:Balanced scaffold + basic feature + supervised}}
%\vspace{-3mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
%\hline
\Xhline{2\arrayrulewidth}
Methods                    & \textbf{BBBP}                           & \textbf{BACE}                           & \textbf{TOX21}                          & \textbf{TOXCAST}                        & \textbf{SIDER}     &    \textbf{AVE GAIN}                       \\ 
%\hline
\Xhline{2\arrayrulewidth}
\nopretrain            & 91.46($\pm$ 0.85) &  84.29($\pm$ 3.80) &  78.35($\pm$ 0.95)  & 68.31($\pm$ 1.61) & 61.15($\pm$ 2.46) & 0($\pm$ 1.934) \\
%\masktask                & 91.23($\pm$ 1.51) & 84.97($\pm$ 1.55) & 77.77($\pm$ 1.23) & 68.98($\pm$ 1.11) & 61.20($\pm$ 0.41)  \\
%\contexttask             & 92.13($\pm$ 1.04) & 84.83($\pm$ 3.19) & 78.79($\pm$ 2.52) & 68.29($\pm$ 1.23) & 62.32($\pm$ 2.99) \\
\supervisedtask              & 90.70($\pm$ 0.74)  & 84.22($\pm$ 2.69) & 80.45($\pm$ 1.47) & 69.47($\pm$ 1.06) & \textbf{63.38($\pm$ 1.44)} & 0.932($\pm$ 1.480)\\
\supervisedmasktask     & 91.10($\pm$ 2.88)  & 85.54($\pm$ 4.57) & \textbf{81.49($\pm$ 1.52)} & 70.77($\pm$ 1.00)  & 62.81($\pm$ 2.61) & 1.630($\pm$ 2.516)\\
\supervisedcontexttask & \textbf{91.54($\pm$ 3.52)} & \textbf{85.71($\pm$ 2.92)} & 81.23($\pm$ 1.94) & \textbf{71.36($\pm$ 1.05)} & 62.75($\pm$ 2.27) & 1.806($\pm$ 2.340)\\ 
%\hline
\Xhline{2\arrayrulewidth}
%\vspace{-10mm}
\end{tabular}
}
\end{table*}
%\vspace{-3mm}
\paragraph{GNN Backbone} The GNN architecture also plays a role in graph pretraining. In~\citet{hu2019strategies}, the results show that pretraining on GNN variants like GIN~\citep{xu2018powerful} would improve the performance on downstream tasks, while the performance with architectures like GAT~\citep{velivckovic2017graph} would actually get worse performance with pretraining. As the GNNs based on 1-Weisfeiler-Lehman (WL) test have similar representation power~\citep{xu2018powerful} bounded by the Weisfeiler-Lehman isomorphism check~\citep{shervashidze2011weisfeiler}, we consider the two representative GNN architectures, namely the \textbf{GIN}~\citep{xu2018powerful} and \textbf{GraphSage}~\citep{hamilton2017representation}. They have shown benefits with graph pretraining in ~\citet{hu2019strategies}.
%\vspace{-3mm}
\paragraph{Pretraining dataset} In natural language pretraining, researchers observed a significant performance boost due to self-supervised pretraining on large-scale data, that is, the larger the pretraining dataset is, the better the downstream performance it is ~\citep{raffel2019exploring}. %We hope to obtain similar outstanding performance improvement as a result of pretraining with large scale datasets for graph pretraining. 
Inspired by this success in natural language processing, we test the algorithms on two unlabeled pretraining datasets with different scales.

\begin{itemize}[noitemsep,topsep=1pt,parsep=1pt,partopsep=0pt, leftmargin=*]
	\item \textbf{ZINC15~\citep{sterling2015zinc}}: ZINC15 contains 2 million molecules. This dataset was preprocessed following ~\citet{hu2019strategies}.
	\item \textbf{SAVI ~\citep{patel2020synthetically}}: The SAVI dataset contains about 1 billion molecules, which are significantly larger than ZINC15. To the best of our knowledge, it has never been used for pretraining tasks before. This dataset contains drug-like molecules synthesized by computer simulated reactions. 
	\end{itemize}

Additionaly, we used \textbf{ChEMBL~\citep{gaulton2012chembl}} as the supervised datasets. Different from the above ZINC15 and SAVI dataset which are only used for self-supervised pretraining, this dataset contains 500k drug-able molecules with 1,310 prediction target labels from bio-activity assays for drug discovery. Thus like in~\citet{hu2019strategies} we only leverage it for \emph{supervised} pretraining. 
%\vspace{1mm}
%\vspace{-4.5mm}
% \paragraph{Pretraining objective} In \Secref{sec:gnn_pretrain} we have provided a brief literature review over the pretraining methods for molecule representation learning. Here we categorize these into objectives with different principles, and consider the representative one per each objective categories. 
% \begin{itemize}
% 	\item \textbf{Masking.} We leverage the \textbf{Node Prediction} objective, which randomly mask 15\% of the nodes' features and then ask GNN to make predictions on the node attributes for the masked ones. This strategy is from~\citet{hu2019strategies} and resembles the BERT pretraining~\citep{devlin2018bert} for natural language.
% 	\item \textbf{Structured.} Unlike text data where the topology is a sequence, the graph has rich structure information. Following~\citet{hu2019strategies} we use \textbf{Context Prediction}, which masks out the context from $k_1$-hops to $k_2$-hops and leverages  adversarial training to let the GNN predict the true context embeddings from the random context embeddings. 
% 	\item \textbf{Graph-level self-supervised.} We ask the GNN to predict the motif it contains. The motif can be extracted from the molecule with RDKit~\citep{landrum2016rdkit}. We denote it as \textbf{Motif Prediction}, and use the same set of 85 motifs~\footnote{\url{http://rdkit.org/docs/source/rdkit.Chem.Fragments.html}} as~\citep{rong2020self} for multi-label classification. 
% 	\item \textbf{Contrastive.} We leverage the \textbf{Contrastive Learning} approach in ~\citep{you2020graph} to corrupt the input node features with Gaussian noise, and leverage the locally normalized probability to maximize the consistency between positive pairs and minimize that between negative pairs.
% 	\item \textbf{Graph-level supervised.} Finally when applicable, we use the ChEMBL dataset with graph-level labels for graph-level \textbf{Supervised Pretraining}, as presented in ~\citet{hu2019strategies}. 
% \end{itemize}
% The above four components are the design choices for pretraining stage. In addition to these stages, we believe the factors in downstream applications can potentially affect the effectiveness of pretraining as well. So we also consider the configurations for the finetuning stages in the downstream tasks. 
% \vspace{-2.0 mm}
\paragraph{Data split on downstream tasks} The downstream tasks for molecular domain we used are 5 benchmark datasets from MoleculeNet~\citep{wu2018moleculenet} (See Appendix~\ref{sec:molecular_benchmarks} for more details). The train/valid/test sets are split with ratio 8:1:1. For molecule domain, the random split is not the most meaningful way to assess the performance, because the real-world scenarios often require generalization ability on out-of-distribution samples. So we consider the following ways to split the data:
\begin{itemize}[noitemsep,topsep=1pt,parsep=1pt,partopsep=0pt, leftmargin=*]
	\item \textbf{Scaffold Split~\citep{hu2019strategies, ramsundar2019deep}} This strategy first sorts the molecules according to the scaffold (e.g. molecule structure), and then partition the sorted list into train/valid/test splits consecutively. Therefore, the molecules in train and test sets are most different ones according to their molecule structure.  Note this strategy would yield deterministic data splits.
	\item \textbf{Balanced Scaffold Split~\citep{bemis1996properties, rong2020self}} This strategy introduces the randomness in the sorting and splitting stages above, thus one can run on splits with different random seeds and report the average performance to lower the evaluation variance.
\end{itemize}

We choose balanced scaffold as our major evaluation configuration, because it allows us to evaluate the algorithm on multiple data splits while maintaining the ability to evaluate out of distribution samples (e.g. assess generalization ability). Evaluating on one single split (such as scaffold split) can be subject to bias due to one specific split, leading to higher variance in evaluation. 
%\vspace{-3mm}
%x
\begin{table*}[t]
\small
%\vspace{-3mm}
\centering
\caption{Unsupervised + \textbf{Basic feature + Scaffold}. No pretrain has an average accuracy of 68.7\% over all benckmark datasets. \label{tab:Scaffold + basic feature + unsupervised}}
%\vspace{-3mm}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
\Xhline{2\arrayrulewidth}
%\hline
Methods               & \textbf{BBBP}                & \textbf{BACE}             & \textbf{TOX21}            & \textbf{TOXCAST}              & \textbf{SIDER} &    \textbf{AVE GAIN}    \\ 
%\hline
\Xhline{2\arrayrulewidth}
\nopretrain              & 69.62($\pm$ 1.05)            & 75.77($\pm$4.29)          & 75.52($\pm$0.67)          & 63.67($\pm$0.32)              & 59.07($\pm$1.13)  &   0($\pm$1.492)\\
\masktask                & 68.70($\pm$2.16)             & 76.95($\pm$0.12)          & 75.88($\pm$0.60)          & 64.11($\pm$0.38)              & 61.29($\pm$0.87)  &   0.656($\pm$0.826)\\
\contexttask             & 69.41($\pm$1.44)             & \textbf{81.96}($\pm$0.72)          & 75.49($\pm$0.75)          & 63.48($\pm$0.31)              & \textbf{62.27($\pm$0.90)}  &   1.792($\pm$0.824)\\
%\supervisedtask          & 68.96($\pm$0.64)             & 76.30($\pm$1.30)          & 76.64($\pm$0.39)          & 66.07($\pm$0.22)              & 61.97($\pm$0.96) \\
%\supervisedmasktask      & \textbf{71.41($\pm$0.67)}    & 84.59($\pm$0.35)          & 79.13($\pm$0.29)          & 65.32($\pm$0.37)              & 62.12($\pm$0.19) \\
%\supervisedcontexttask   & 69.63($\pm$0.25)             & \textbf{83.34($\pm$0.67)} & 78.11($\pm$0.28)          & 66.15($\pm$0.48)              & 63.48($\pm$0.43) \\ 
%\hline
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\end{table*}


\begin{table*}[t]
% \small
%\vspace{-5mm}
\centering
\caption{Supervised + \textbf{Basic feature + Scaffold}. No pretrain has an average accuracy of 68.7\% over all benckmark datasets. \label{tab:Scaffold + basic feature + supervised}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
%\hline
\Xhline{2\arrayrulewidth}
Methods                & \textbf{BBBP}                & \textbf{BACE}             & \textbf{TOX21}            & \textbf{TOXCAST}              & \textbf{SIDER}   &    \textbf{AVE GAIN}  \\ 
%\hline
\Xhline{2\arrayrulewidth}
\nopretrain              & 69.62($\pm$ 1.05)            & 75.77($\pm$4.29)          & 75.52($\pm$0.67)          & 63.67($\pm$0.32)              & 59.07($\pm$1.13)   &  0($\pm$1.492)\\
%\masktask                & 68.70($\pm$2.16)             & 76.95($\pm$0.12)          & 75.88($\pm$0.60)          & 64.11($\pm$0.38)              & 61.29($\pm$0.87) \\
%\contexttask             & 69.41($\pm$1.44)             & 81.96($\pm$0.72)          & 75.49($\pm$0.75)          & 63.48($\pm$0.31)              & 62.27($\pm$0.9)  \\
\supervisedtask          & 68.96($\pm$0.64)             & 76.30($\pm$1.30)          & 76.64($\pm$0.39)          & 66.07($\pm$0.22)              & 61.97($\pm$0.96)  &   1.258($\pm$0.702)\\
\supervisedmasktask      & \textbf{71.41($\pm$0.67)}    & 84.59($\pm$0.35)          & \textbf{79.13($\pm$0.29)} & 65.32($\pm$0.37)              & 62.12($\pm$0.19) &    3.784($\pm$0.374)\\
\supervisedcontexttask   & 69.63($\pm$0.25)             & \textbf{83.34($\pm$0.67)} & 78.11($\pm$0.28)          & \textbf{66.15($\pm$0.48)}     & \textbf{63.48($\pm$0.43)} &   3.412($\pm$0.422)\\ 
%\hline
\Xhline{2\arrayrulewidth}
%\vspace{-12mm}
\end{tabular}

}
\end{table*}
\subsection{Experiment protocol}
\label{sec:protocol}
As the total number of configurations for the entire pipeline can be combinatorially large which is not practical for us to exhaustively experiment with all of them, we design our protocol with a pairwise comparison principle. Specifically, we first anchor a \emph{vanilla configuration} with a certain design choice of combination for each stage. To study the effect of each stage on the pretraining effectiveness, we vary the design choice one stage at a time compared to the \emph{vanilla configuration}. %In total we would run $N$ sets of experiments where $N$ is the number of varying stages we considered. Note that in each set of experiments we will still have multiple experiments for each possible design choices we consider for that stage.

%By pairwise comparison between each set of variations and the \emph{vanilla configuration}, we can see how the design choices affect the outcome of the pretraining, and in which scenario will the pretraining help most for the downstream tasks. However, whenever feasible, we can also analyze the effect of joint variations on multiple stages by comparing the results of them together. We will present these results, our analysis and hypothesis in the next section. 

For all these experiments, to assess the effectiveness of graph pretraining, we report the \textbf{ROC-AUC} on downstream tasks as well as the relative \textbf{average gain} over all downstream datasets with and without pretraining. For each setting we will report the mean and standard deviation (in parenthesis) over three runs with different random seeds. We tune the model on downstream tasks with the validation set, and report the evaluation metric on the test set using the model with best validation performance. For each setup, we report the average performance obtained with three random seeds. We tune the learning rate in $\{1e^{-4}, 5e^{-4}, 1e^{-3}, 5e^{-3}, 1e^{-2}, 5e^{-2}, 1e^{-1}\}$ for each setup \emph{individually} and select the one with best validation performance. For GNNs we fix the hidden dimension to 300 and number of layers to 5.

==> [NeurIPS2022-axive]Does GNN Pretraining Help Molecular Representation_/gnn_pretrain.tex <==
\section{Preliminary}
\label{sec:gnn_pretrain}

\input{summary_table}

%\section{Graph Pretraining}
%Some data like chemical molecules contains structure information, which can be modeled as a graph. For example, in chemical molecules, atoms are modeled as nodes, and bonds are modeled as edge. Start from some format of node and edge feature, Graph neural networks performs several rounds of convolution of every node using the features of its connected neighbour nodes and the edges between them. After several sounds of convolution, the node feature and edge feature are Therefore, it is a natural way to represent raw format of data into deep-learning usable representation while maintain structure information.  THe representation can be used on pretraining tasks or downstream tasks with different objectives. 
% {\color{red} In graph learning, there
% are usually two categories of supervised tasks: i) Node classification/regression, where each node
% v has a label/target yv, and the task is to learn to predict the labels of unseen nodes; ii) Graph
% classification/regression, where a set of graphs {G1, ..., GN } and their labels/targets {y1, ..., yN } are
% given, and the task is to predict the label/target of a new graph.

% %we divide existing graph SSL methods into three categories: contrastive, generative, and predictive,

% }

%We choose implementation of ICLR paper \citet{hu2019strategies}, as we can reproduce the results reported in the paper, and we can observe gains on the proposed scaffold split under the authors setup. 

\paragraph{Graph Neural Networks (GNNs).} Let $G = \{V, E\}$ denote a molecule graph with $V$ as the set of nodes and $E$ as the set of edges. 
%$X_v$ as node attributes for $v \in V$ and $e_{ij}$ as edge features for edge(i, j) $\in E$. 
Given the node features $X_i$, most GNNs learn an embedding representation $h_i$ for every node $i \in V$ by aggregating representations from connected nodes and edges, denoted as graph convolution. These procedure repeats for $K$ times with the update equation as follows:
\begin{equation}
%\resizebox{1.0\hsize}{!}{$
h_i^k = \text{UPDATE}(h_i^{k-1}, \text{AGGREGATE}(\{h_i^{k-1}, h_j^{k-1}, e_{ij}\}: \forall j \in N(i))) \nonumber
%$}
\end{equation}
where $\gN(i)$ is the set of neighbor nodes of $i$ and $h_i^0 = X_i$. The representation for entire graph $G$ is then obtained by permutation-invariant transformation on node representation,  $h_G = \text{READOUT}(h_i^K | i\in V)$. In this paper we mainly study the GNNs that belong to this family, namely the WL-1 GNNs.

\paragraph{Finetune.} After the pretraining, the pretrained model is used to finetune on the downstream tasks. For molecule property prediction tasks, the graph-level representation obtained from the pretrained model is connected to linear classifiers to predict downstream task labels. The fine-tuning is performed in an end-to-end manner, where both the pretrained GNN and the linear classifiers are trainable. %: $y_G = f_F(h_G)$, where $h_G = \text{GNN}_{\theta}(X_G)$. the notation is terrible, so I'll just delete these for simplicity.

\paragraph{Graph pretraining objectives.} The primary goal of pretraining is to learn representations with robust transferable knowledge of graphs from the abundant pretraining data %through well-designed pretraining objectives. The learned knowledge can be 
and then generalize to downstream tasks with usually different supervision signals. Generally the pretraining objectives can be categorized into self-supervised and 
supervised ones. We present a brief overview of some representative objectives in the following sections. 

\subsection{Self-supervised (unsupervised) pretraining}
In self-supervised pretraining, the pretraining objective is designed to learn self-generated targets from the structure of the molecules, such as the type of nodes and edges, prediction of local context, graph partition, node clustering, occurrence of some functional groups, and etc. The predictive target can be node/edge level or entire graph level. We present some representative ones below:

{\color{red} %e both node and graph embeddings are of high-quality so that graph embeddings are robust and transferable across downstream tasks

%Therefore, while this type of pre-training is also very natural, it is beyond the scope of this paper and we leave its investigation for future work.

% When the GNN pre-training is finished, we fine-tune the pre-trained GNN model on downstream tasks. Specifically, we add linear classifiers on top of graph-level representations to predict downstream graph labels. The full model, i.e., the pre-trained GNN and downstream linear classifiers, is subsequently fine-tuned in an end-to-end manner. 

}
\subsubsection{Node Prediction}
Node prediction is a node-level classification task given the masked context of entire graph. Similar to \citet{devlin2018bert}, some portion of node attributes are masked and replaced with mask-specified indicators in the node input feature. After graph convolution, %aggregating neighbor representations, 
the embedding output from GNN is used to predict the true attribute of the node, e.g. atom type in molecular graphs, through a linear classifier on top of the node embedding. 
%The training objective is % $\min \sum_i \text{loss}(f_N(h_i), T_i)$ where $GNN$
%the   The node attribute is masked and the pretraining GNN is to predict the type of node (atom) 
%\cite{devlin2018bert}
%{\color{red} In Attribute Masking, we aim to capture domain knowledge by learning the regularities of the node/edge attributes distributed over graph structure.  Attribute Masking pre-training works as follows: We mask node/edge attributes and then we let GNNs predict those attributes (Devlin et al., 2019) based on neighboring structure.  Specifically, We randomly mask input node/edge attributes, for example atom types in molecular graphs, by replacing them with special masked indicators. We then apply GNNs to obtain the corresponding node/edge embeddings (edge embeddings can be obtained as a sum of node embeddings of the edge’s end nodes). Finally, a linear model is applied on top of embeddings to predict a masked node/edge attribute. }
%\begin{equation}
%   \min_{\theta, \gamma} \sum_i \text{Loss}(f_{N_\gamma}(h_i), T_i ) \quad \text{where } h_i = \text{GNN}_{\theta}(X_i)  
% \end{equation}


\subsubsection{Context Prediction}
Context prediction task is a sub-graph level task aiming at learning embedding that can represent the local subgraph surrounding a node. Generally it can be viewed as a masked task for substructure. Since it is essentially a structured prediction which can be difficult in general, \citet{hu2019strategies} leverages the adversarial learning to teach the model to distinguish the positive sub-graph embedding from the negative ones. 
%dot product of the two embedding. 
\citet{rong2020self} instead builds a dictionary of structures that captures the property of sub-graphs (e.g. type and quantity of neighbour nodes and bonds), and turns it into a multi-class classification problem. %using the embedding of node in the context center. %$h_i^K$. 
% {\color{red} In Context Prediction, we use subgraphs to predict their surrounding graph structures. Our goal
% is to pre-train a GNN so that it maps nodes appearing in similar structural contexts to nearby embeddings. 
% \textbf{GROVER} For the node/edge-level
% tasks, instead of predicting the node/edge type alone, GROVER randomly masks a local subgraph
% of the target node/edge and predicts this contextual property from node embeddings.
% The prediction target should reflect contextual information of the node/edge. Guided by these
% criteria, we present the tasks on both nodes and edges.
% They both try to predict the context-aware properties of
% the target node/edge within some local subgraph. 
% }
%\begin{equation}
%    % \quad
%    \min_{\theta} \sum_i \text{loss}(C_i, h_i) \quad \text{where } 
%    \quad
%    C_i = f_C(h_i, h_j: j\in \text{context}(i))
%\end{equation}
%where $f_c$ performs some transformation on context and target node to generate context embedding or labels. $f_C$ is embedding extraction function for \cite{hu2019strategies} and is label extraction for \cite{rong2020self}.

\subsubsection{Motif Prediction}
Motif prediction~\citep{rong2020self} is to %learn graph-level embedding through 
predict the existence of functional groups, such as benzene ring or hydroxyl. The motifs are extracted automatically from RDKit~\citep{landrum2016rdkit} . The motif prediction task is formulated as a graph-level multi-label binary classification task, where the graph embedding is used to jointly predict the occurrence of these semantic functional motifs.  %with one label for one motif. 
%Given a molecule, computational sorftware  can provide the supervised labels, and one label for one motif. Hence motif prediction task is a self-supervised task. The training objective is   
%
%\begin{equation}
%   \min_{\theta, \omega}  \text{Loss}(f_{M_\omega}(h_G), \{M_j: j = 1,2, .. m \} ) \quad \text{where } h_G = \text{GNN}_{\theta}(X) 
% \end{equation}
%where  $\{M_j: j = 1,2, .. m \}$ is a set of binary labels for $m$ motifs. $f_{M_\omega}$ is a multi-task linear classifier parameterized by $\omega$. 
 

%{\color{red} For the graph-level tasks, by incorporating the domain knowledge, GROVER extracts
%the semantic motifs existing in molecular graphs and predicts the occurrence of these motifs for a molecule from graph embeddings.

%fs are recurrent sub-graphs among the input graph data, which are prevalent in molecular graph data. One important class of motifs in molecules are functional groups, which encodes the rich domain knowledge of molecules and can be easily detected by the professional software, such as RDKit [27]. Formally, the motif prediction task can be formulated as a multi-label classificationproblem, where each motif corresponds to one label. }
\subsubsection{Contrastive learning}
Graph contrastive learning is to %, pretraining is performed through
maximize the agreement of two augmented views of the same graph, and minimize the agreement of different graphs. The optimization is conducted using contrastive loss in the latent embedding space \citep{you2020graph, hassani2020contrastive,zhu2021graph,wu2021self}. The augmentation function needs to transform graphs into realistic and novel augmentations without affecting semantic labels of the graphs. For example, the transformation can be small perturbations or modifications on node/edge embedding, drop of a few nodes or edges, and so on. These transformations enforce an underlying prior for contrastive learning, that is, local transformation does not change the semantic meaning of a graph.
%\begin{equation}
%\min_\theta -sim(h_G, h_G') + sum(h_G, h_G'') 
%\end{equation}
%\begin{equation}
%\text{where  } G'=f_A(G), G''=f_A(G_1), G1 \neq G
%\end{equation}
%where $sim$ is some similarity measure like cosine similarity. 

%The underlying prior enforced by it is that missing part of vertices does not affect the semantic meaning of



% {\color{red}

%  The main idea of contrastive learning is to make representations agree with
% each other under proper transformations, raising a recent surge of interest in visual representation
% learning

% In graph contrastive learning, pre-training is performed through maximizing the agreement
% between two augmented views of the graph via a contrastive loss in the latent space a

% contrastive learning aims to learn one or
% more encoders such that representations of similar graph
% instances agree with each other, and that representations
% of dissimilar graph instances disagree with each other. W

% }


% . A contrastive loss function L(·) is defined to enforce maximizing
% the consistency between positive pairs zi
% , zj compared with negative pairs. Here we utilize the
% normalized temperature-scaled cross entropy loss (NT-Xent) [51, 25, 52].
% During GNN pre-training, a minibatch of N graphs are randomly sampled and processed through
% contrastive learning, resulting in 2N augmented graphs and corresponding contrastive loss to optimize,
% where we re-annotate zi
%  zj as zn i  zn j for the nth graph in the minibatch. Negative pairs are not
% explicitly sampled but generated from the other N − 1 augmented graphs within the same minibatch
% as in [53, 18]. Denoting the cosine similarity function as sim(zn,i, zn,j ) = z
% T
% n,izn,j/kzn,ikkzn,jk,
% NT-Xent for the nth graph is defined as:
%  n = −log exp(sim(zn i, zn j )/tau )
% PN
% n0=1,n06=n
% exp(sim(zn,i, zn0
% ,j )/tau)
% , (3)
% where τ denotes the temperature parameter. The final loss is computed across all positive pairs in the
% minibatch. The proposed graph contrastive learning is summarized in Appendix A.}
%\vspace{-1mm}
\subsection{Supervised pretraining}
%{\color{red} We inject graph-level domain-specific knowledge into our pretrained embeddings by defining supervised graph-level prediction tasks In particular, we consider a practical method to pre-train graph representations: graph-level multi-task supervised pre-training to jointly predict a diverse set of supervised labels of individual graphs. }
Supervised pretraining aims to learn domain-specific graph-level knowledge from specifically designed pretraining tasks. For molecular application, the supervised labels are generated from a diverse set of functional studies like biochemical assays. The pretrainning task is to perform multiple binary classification and jointly learn the supervised labels. Although the pretraining mainly refers to unsupervised or self-supervised methods as they are not limited by the requirement of supervised labels, supervised pretraining is still a great source to investigate the graph pretraining in general.


\begin{table*}[t]
\small
\centering
%\vspace{-2mm}
\caption{\textbf{Self-supervised} + Rich feature + Balanced Scaffold Split.  No pretrain has an average value of 78.0\% over all 5 datasets. \label{tab:unsupervised-obj}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
\Xhline{2\arrayrulewidth}
%\hline
Methods           & \textbf{BBBP}            & \textbf{BACE}                  & \textbf{TOX21}           & \textbf{TOXCAST}        & \textbf{SIDER  }  &    \textbf{AVE GAIN}    \\ %\midrule %\hline
\Xhline{2\arrayrulewidth}
\nopretrain      & 92.23($\pm$3.07) & 87.43($\pm$1.63)     & 79.20($\pm$1.99)  & 69.13($\pm$0.55) & 61.92($\pm$0.89) & 0($\pm$1.626)\\
\masktask        & 92.24($\pm$2.76) & 87.32($\pm$1.67)     & 79.57($\pm$2.03) & 69.77($\pm$0.13) & 61.62($\pm$1.12) & 0.122($\pm$1.542)\\
\contexttask     & 92.68($\pm$1.19) & 86.98($\pm$1.26)     & 79.05($\pm$2.51) & 70.18($\pm$0.44) & 61.65($\pm$0.77) & 0.126($\pm$1.234)\\
\motiftask       & 92.63($\pm$1.19) & 87.16($\pm$1.66)     & 79.22($\pm$2.38) & 69.09($\pm$0.07) & 62.45($\pm$1.25) & 0.128($\pm$1.310)\\  
\contrastivetask  & 92.31($\pm$1.58)& 86.67($\pm$2.40)     & 78.45($\pm$2.44) & 68.37($\pm$0.80) & 61.22($\pm$1.20) & -0.578($\pm$1.684) \\ 
%\hline
\Xhline{2\arrayrulewidth}
%\vspace{-6mm}
\end{tabular}%
}
\vspace{-2mm}
\end{table*}

\begin{table*}[h]
\small
%\caption{Supervised Pretraining Objectives on Downstream Task Accuracy (\%)}
%\vspace{-2mm}
\centering
\caption{\textbf{Supervised} + Rich feature + Balanced Scaffold.  No pretrain has an average AUC of 78.0\%. \label{tab:super-obj}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
%\hline
\Xhline{2\arrayrulewidth}
Methods                    & \textbf{BBBP}   & \textbf{BACE}   & \textbf{TOX21}   & \textbf{TOXCAST} & \textbf{SIDER}  &    \textbf{AVE GAIN}   \\ 
\Xhline{2\arrayrulewidth}
\nopretrain      & 92.23($\pm$3.07) & 87.43($\pm$1.63) & 79.2($\pm$1.99)  & 69.13($\pm$0.55) & 61.92($\pm$0.89) & 0($\pm$1.626)\\
\supervisedtask  & 91.65($\pm$2.11) & 86.91($\pm$1.86) & 81.13($\pm$2.39) & 71.64($\pm$0.46) & 62.14($\pm$1.13) & 0.712($\pm$1.590)\\
\supervisedmasktask     & \textbf{93.43($\pm$2.50)} & 86.90($\pm$2.04) & \textbf{81.93($\pm$1.79)} & 71.66($\pm$0.73) & 62.68($\pm$1.82) & 1.338($\pm$1.776)\\
\supervisedcontexttask& 92.27($\pm$1.57) & \textbf{88.72($\pm$1.68)} & 81.71($\pm$1.79)   & \textbf{72.19($\pm$0.79)}  & \textbf{63.21($\pm$1.49)}  & 1.638($\pm$1.464) \\ 
\Xhline{2\arrayrulewidth}
%\vspace{-10mm}
\end{tabular}%
}
\vspace{-2mm}
\end{table*}

\begin{table*}[t]
\small
%\vspace{-3mm}
\centering
\caption{Self-supervised + Rich feature + \textbf{Scaffold}. No pretrain has an average ROC-AUC of 71.8\% over all benckmark datasets. \label{tab:split}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
%\hline
\Xhline{2\arrayrulewidth}
Methods        & \textbf{BBBP}             & \textbf{BACE}    & \textbf{TOX21}    & \textbf{TOXCAST} & \textbf{SIDER} &    \textbf{AVE GAIN}   \\ %\hline
\Xhline{2\arrayrulewidth}
%\nopretrain      & \textbf{75.13($\pm$1.08)} & 79.79($\pm$1.18) &  76.06($\pm$0.20) & 66.1($\pm$0.42)  & 61.21($\pm$0.76) \\
\nopretrain      & 74.83($\pm$0.73) & 80.10($\pm$0.42) & 75.86($\pm$0.58)  & 65.95($\pm$0.15) & 62.30($\pm$1.14) & 0($\pm$0.579)\\
\masktask        & 73.45($\pm$0.27) & 83.66($\pm$0.75) & 75.30($\pm$0.37)  & 66.50($\pm$0.06) & 65.08($\pm$0.12) & 0.990($\pm$0.323)\\
\contexttask     & 74.10($\pm$0.22) & 81.87($\pm$0.49) &75.37($\pm$0.11)   & 66.86($\pm$0.07) & 62.84($\pm$0.46) & 0.400($\pm$0.280)\\
\motiftask       & 73.65($\pm$0.36) & 80.58($\pm$2.04) & 74.55($\pm$0.79)  & 65.63($\pm$0.07) & 64.05($\pm$0.23) & -0.116($\pm$0.766)\\
\contrastivetask & 73.32($\pm$2.38) & 80.51($\pm$0.80) & 74.55($\pm$0.22)  & 65.70($\pm$0.09) & 64.39($\pm$0.63) & -0.114($\pm$0.513)\\ 
%\hline
\Xhline{2\arrayrulewidth}
%\vspace{-6mm}
\end{tabular}%

}
%\caption{Scaffold split + rich feature}
\end{table*}

\begin{table*}[t]
\small
\centering
%\vspace{-3mm}
\caption{Supervised %+ Self-supervised 
+ Rich feature + \textbf{Scaffold}. No pretrain get 71.8\% average ROC-AUC. \label{tab:feature-scaffold-richfeature-supervised}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
%\hline
\Xhline{2\arrayrulewidth}
Methods & \textbf{BBBP}              & \textbf{BACE}     & \textbf{TOX21}    & \textbf{TOXCAST}      & \textbf{SIDER} &    \textbf{AVE GAIN}  \\ %\hline
\Xhline{2\arrayrulewidth}
\nopretrain                 & \textbf{74.83($\pm$0.73)}     & 80.10($\pm$0.42)          & 75.86($\pm$0.58)          & 65.95($\pm$0.15)          & 62.30($\pm$1.14)           & 0($\pm$0.604) \\
\supervisedtask             & 72.79( $\pm$ 0.7)             & 83.23($\pm$0.67)          & 77.66($\pm$0.08)          & 67.72($\pm$0.13)          & 65.34($\pm$0.17)           & 1.540($\pm$0.350) \\
\supervisedmasktask         & 73.38($\pm$0.55)              & \textbf{84.42($\pm$0.27)} & \textbf{77.85($\pm$0.24)} & \textbf{67.14($\pm$0.28)} & 64.06($\pm$0.28)           & 1.562($\pm$0.324) \\
\supervisedcontexttask      & 73.81($\pm$0.52)              & \ 84.35($\pm$0.93)        & 77.11($\pm$0.14)          & 67.87($\pm$0.08)          & \textbf{65.19($\pm$0.17)}  & 1.858($\pm$0.368)  \\ 
%\hline
\Xhline{2\arrayrulewidth}
%\vspace{-7mm}
\end{tabular}%
}
\end{table*}

==> [NeurIPS2022-axive]Does GNN Pretraining Help Molecular Representation_/introduction.tex <==
\section{Introduction}





%The gain obtained by pretraining, mainly refer to supervised pretraining,  is larger in lower accuracy region (i.e. on scaffold split, basic feature) than that on high accuracy region (i.e. on balanced scaffold, rich feature). By using rich features, the gain achieved by supervised pretraining is reduced. 


%We reach a conclusion that unsupervised pretraining strategies do not have significance improvements over no pretraining, whereas supervised pretrainig improves more on low accuracy region, whereas the effect is reduced in higher accuracy region (i.e.achieved by balanced split or rich feature). 

Graph neural networks (GNNs)
, due to their effectiveness,
have been adopted to model a wide range of structured data, such as social networks, road graphs, citation networks, etc. Molecule modeling is one of these important applications, where it serves as the foundation of biomedicine and nurturing techniques like novel drug discovery. However, labeling biomedical data are usually time-consuming and expensive and thus task-specific labels are extremely inadequate. This poses a big challenge to the field. Recently, inspired by the remarkable success of self-supervised pretraining from natural language processing~\citep{devlin2018bert, brown2020language,wei2021finetuned} and computer vision domains~\citep{he2020moco,chen2020simple}, researchers start trying to apply the pretrain-finetune paradigm to molecule modeling with GNN, hoping to boost the performance of various molecular tasks by pretraining the model on the enormous unlabeled data.
% Therefore, self-supervised pretraining is indeed very attractive as it might potentially alleviate this issue.
% In this paper, we are particularly interested in the GNN pretraining for molecule presentations. 
% The past few years have witnessed the remarkable achievements of self-supervised pretraining in many scientific fields, such as computer vision \adamsyuwei{should cite Kaiming He "Moco" and Ting Chen "SimCLR"} \citep{dosovitskiy2020image,dai2021coatnet,chen2020simple} and natural language processing \adamsyuwei{should cite Jacob Devlin "BERT"} \citep{raffel2019exploring, wei2021finetuned,brown2020language}. Recently, researchers start trying to apply the pretrain-finetune paradigm to other less explored domains with abundant unlabeled data, hoping to replicate the success of self-supervised pretraining.
% exploiting opportunities to accelerate the process of transferring robust generalizable knowledge obtained from abundant pretraining data to benefit realistic tasks in drug discovery and biomedical domain (molecules).
% Molecules are usually abstracted as graphs to preserve its rich structure information. Self-supervised graph pretraining is of particular interest because: First, task-specific labels are inadequate, as biomedical labeling requires time and resource-intensive wet-lab experiments, and pretraining can be a good option to alleviate the issue as it is in computer vision \citep{chen2020simple,sohn2020fixmatch}; Second, models suffer from poor generalization capability in chemical space. Pretraining can initialize graph neural networks models to a ``better'' basin around a good local optima that can better generalize. % Encouraging results [cite??] have been reported recently on the efficacy of GNN pretraining in molecule representation, claiming downstream applications indeed benefit from finetuning the pretrained networks.
For instance, %a large variety of 
many methods have been proposed~\citep{xie2021self,wu2021self}, where significant performance improvements are claimed
% due to well designed pretraining objectives and 
by pretraining on large scale datasets \citep{hu2019strategies, rong2020self,  you2020graph, you2020does, zhu2021graph}. Despite of the promising results, %we find research on investigating the factors for the improvement are still at a nascent stage. Based on our experiments, 
we find that reproducing some of these outstanding gains via graph pretraining can be non-trivial, and sometimes the improvement largely relies on the experimental setup and the extensive hyper-parameter tuning of downstream tasks, rather than the design of pretraining objectives. These observations motivate us to rethink the effectiveness of graph pretraining with unsupervised or self-supervised objectives, and investigate what factors would influence the effectiveness of self-supervised graph pretraining.
% and to investigate what possibly influences the effectiveness. % All of these motivate this paper.

\begin{figure*}[ht]
\includegraphics[width=1.0\textwidth]{figs/graph_pretrain_pipeline.drawio_morestraws}
\caption{A typical pipeline for graph pretraining and deployment for downstream applications. \label{fig:pipeline}}
\end{figure*}


In this paper, we perform systematic studies to
assess the performance of popular graph pretraining objectives on different types of datasets, and exploit various confounding components in experimental setup in deciding the performance of downstream tasks with or without pretraining. 
Here, we restrict our studies to small molecular graphs, as opposed to other application domains, such as social networks or citation graphs. The key insights and take-aways of this paper are:
\begin{itemize}[leftmargin=*]%[noitemsep,topsep=1pt,parsep=1pt,partopsep=0pt, leftmargin=*]
    \item Among the pretraining tasks we evaluated, the self-supervised pretraining alone does not provide statistically significant improvements over non-pretrained methods on downstream tasks.
    \item When additional supervised pretraining step is conducted after self-supervised pretraining, we observe statistically significant improvements. However, the gain becomes marginal on some specific data splits or diminishes if richer features are introduced.
    \item Beyond data splits and hand-crafted features, the usefulness of graph pretraining is also sensitive to the experimental hyperparameters, such as learning rates and number of study repeats. Different setups can lead to opposite conclusions. 
    \item In conclusion, different from the previous works, we do not observe clear and unconditional gains achieved by graph pretraining on molecular representation, indicating it is still too early to conclude graph pretraining is effective in molecular domain.
    \item  We investigate the reason of above and hypothesize that the complexity of some pretraining methods on molecules is insufficient, leading to less transferable knowledge for downstream tasks.
\end{itemize}

Despite the overall negative results we obtained, the main goal of this paper is not to discourage the pretraining research for small molecules. Instead, we hope to raise the attention on different aspects of experiments and the role of simple hand-crafted features, so as to provide useful information for designing better pretraining approaches. Below we first introduce the background of GNN and its pretraining in \secref{sec:gnn_pretrain}, and then our experimental design and results in \secref{sec:exp_framework} and \secref{sec:results}, respectively. Finally we conclude with our findings and the limitations in \secref{sec:summary} and  \secref{sec:limitation}.
% \begin{itemize}[noitemsep,topsep=1pt,parsep=1pt,partopsep=0pt, leftmargin=*]
%     \item Model: we choose GIN
%     \item Pretraining datatset: Zinc
%     \item scaffold: we use balanced scaffold, as ...
% \end{itemize}

% Systematic study is performed to
% assess the performance of contrasting different augmentations on various types of datasets, revealing
% the rationale of the performances and providing the guidance to adopt the framework for specific
% datasets. 



% However, the effectiveness of these methods remains unclear. The authors found to reproduce some of the reported large gain of graph pretraining results are non-trivial, if not unlikely. The good performance of downstream is largely relied on extensive hyper parameters tuning, which 

% %The main goal of this study was therefore to compare the performance of proposed graph pretraining methods and 


% %Grover \citep{rong2020self}

% %ICLR \citep{hu2019strategies}


% The insights
% we gained are that well-designed self-supervision losses and largely-expressive
% pre-trained models enjoy the significant potential on performance boosting.


% Existing work claims: The success of the pre-training model crucially depends on the design of self-supervision tasks.

% Molecules can be naturally represented as graph to preserve rich structure information,  graph-pretraining on molecule domain has raised surge of interest and many promising 

% The robust transferable knowledge learned from the abundant pretraining data generalize to other downstream tasks of interest 
% {\color{red}
% [\textbf{good sentences copied from other paper, rephrase!}] \\


% Inspired by the remarkable achievements of deep learning in many scientific domains, such as computer vision, natural language processing, and social networks, researchers
% are exploiting deep learning approaches to accelerate the process of drug discovery and reduce costs
% by facilitating the rapid identification of molecules. Molecules can be naturally represented by
% molecular graphs which preserve rich structural information. Therefore, supervised deep learning of
% graphs, especially with Graph Neural Networks(GNNs) have shown promising results in
% many tasks, such as molecular property prediction and virtual screening.


% Despite the fruitful progress, two issues still impede the usage of deep learning in real scenarios:
% (1) insufficient labeled data for molecular tasks; (2) poor generalization capability of models in the
% enormous chemical space. Different from other domains (such as image classification) that have
% rich-source labeled data, getting labels of molecular property requires wet-lab experiments which is
% time-consuming and resource-costly. As a consequence, most public molecular benchmarks contain
% far-from-adequate labels. Conducting deep learning on these benchmarks is prone to over-fitting and
% the learned model can hardly cope with the out-of-distribution molecules.

% Recently, GNNs have received a surge of interest in various
% domains, such as knowledge graph, social networks and drug discovery.

% Generalizable, transferrable, and robust representation learning on graph-structured
% data remains a challenge for current graph neural networks (GNNs). Unlike what
% has been developed for convolutional neural networks (CNNs) for image data,
% self-supervised learning and pre-training are less explored for GNNs. In this
% paper, we propose a graph contrastive learning (GraphCL) framework for learning
% unsupervised representations of graph data. W

% The results show that, even without tuning augmentation
% extents nor using sophisticated GNN architectures, our GraphCL framework can
% produce graph representations of similar or better generalizability, transferrability,
% and robustness compared to state-of-the-art methods. 

% We however argue for the necessity of exploring GNN pre-training schemes. Task-specific labels
% can be extremely scarce for graph datasets (e.g. in biology and chemistry labeling through wet-lab
% experiments is often resource- and time-intensive) [15, 9], and pre-training can be a promising
% technique to mitigate the issue, as it does in convolutional neural networks (CNNs) [16, 17, 18]. As to
% the conjectured reasons for the lack of GNN pre-training: first, real-world graph data can be huge and
% even benchmark datasets are recently getting larger [12, 19]; second, even for shallow models, pretraining could initialize parameters in a “better" attraction basin around a local minimum associated
% with better generalization [11]. Therefore, we emphasize the significance of GNN pre-training.

% In comparison, contrastive
% learning aims to learn representations by maximizing feature consistency under differently augmented
% views, that exploit data- or task-specific augmentations [33], to inject the desired feature invariance.

% as graphs are abstracted representations of raw data with
% diverse nature (e.g. molecules made of chemically-bonded atoms and networks of socially-interacting
% people). It is thus difficult to design a GNN pre-training scheme generically beneficial to down-stream
% tasks.

% overcome the aforementioned
% limitations of proximity-based pre-training methods

% h imposes certain prior
% over graph data and parameterized for the extent and pattern. (ii) Utilizing them to obtain correlated
% views, we propose a novel graph contrastive learning framework (GraphCL) for GNN pre-training, 

% Systematic study is performed to
% assess the performance of contrasting different augmentations on various types of datasets, revealing
% the rationale of the performances and providing the guidance to adopt the framework for specific
% datasets. 

% Utilizing them to obtain correlated
% views, we propose a novel graph contrastive learning framework (GraphCL) for GNN pre-training, so
% that representations invariant to specialized perturbations can be learned for diverse graph-structured
% data.



% The main idea of contrastive learning is to make representations agree with
% each other under proper transformations, raising a recent surge of interest in visual representation
% learning [45, 25, 26, 27, 18]. On a parallel note, for graph data, traditional methods trying to
% reconstruct the adjacency information of vertic

% %Data augmentation aims at creating novel and realistically rational data through applying certain transformation without affecting the semantics label. I

% graph datasets are abstracted from diverse fields and therefore there may not be universally
% appropriate data augmentation as those for images.

% node dropping will randomly discard certain portion of vertices

% s the challenge of data heterogeneity in graphs.

% contrastive learning has renewed a surge of interest

% Motivated by recent contrastive learning developments in visual representation learning 

% %In graph contrastive learning, pre-training is performed through maximizing the agreement
% %between two augmented views of the same graph via a contrastive loss in the latent space a

% Therefore, a well designed pre-training
% framework is needed to capture highly heterogeneous information in graph-structured data.

%  It implies that the semantic meaning of G
 


% several works aim to establish a pre-trained model directly on the graph
% representations of molecules.


% An effective approach to this
% challenge is to pre-train a model on related tasks where data is abundant, and then
% fine-tune it on a downstream task of interest. 

% While pre-training has been effective
% in many language and vision domains, it remains an open question how to effectively use pre-training on graph datasets. 

% graph
% data from real-world applications often contain out-of-distribution samples, meaning that graphs in
% the training set are structurally very different from graphs in the test set. Out-of-distribution prediction
% is common in real-world graph datasets


%  The key idea is to use easily accessible
% node-level information and encourage GNNs to capture domain-specific knowledge about nodes and
% edges, in addition to graph-level knowledge. This helps the GNN to learn useful representations
% at both global and local levels




% Recently self-supervised learning (SSL) techniques have gained success in many domains, e.g., visual, natural language processing, and robotics, where SSL methods even outperform their supervised counterparts. However, the development of SSL in the graph domain is still at a nascent stage.

% achieved remarkable success

% Based on how the pretext training tasks are designed,
% SSL methods can be divided into two categories; namely
% contrastive models and predictive models. The major difference between the two categories is that contrastive models
% require data-data pairs for training, while predictive models
% require data-label pairs, where the labels are self-generated
% from the data




% To alleviate this issue, the key insight 

% the combined strategy produces much more transferable graph representations and robustly improves
% downstream performance 


% How to obtain informative representations of molecules is a crucial prerequisite
% in AI-driven drug design and discovery. Recent researches abstract molecules as
% graphs and employ Graph Neural Networks (GNNs) for molecular representation
% learning. Nevertheless, two issues impede the usage of GNNs in real scenarios:
% (1) insufficient labeled molecules for supervised training; (2) poor generalization
% capability to new-synthesized molecules. To address them both, w

% can learn rich structural and semantic information of molecules from enormous unlabelled molecular data.

% The insights
% we gained are that well-designed self-supervision losses and largely-expressive
% pre-trained models enjoy the significant potential on performance boosting.


% Existing work claims: The success of the pre-training model crucially depends on the design of self-supervision tasks.

% abundant labeled data,

% d, as advocated in  



% The
% primary goal of SSL is to learn transferable knowledge from
% abundant unlabeled data with well-designed pretext tasks
% and then generalize the learned knowledge to downstream
% tasks with specific supervision signals.

% Inevitably,
% such divergence will significantly hurt the generalization of
% learned models. Therefore, it is crucial to reconsider the objectives of pretext tasks to better match that of downstream
% tasks and make them consistent with each other.

%  The main idea of contrastive learning is to make representations agree with
% each other under proper transformations, raising a recent surge of interest in visual representation
% learning

% }



% \begin{itemize}
%     \item Pretraining \& success
%     \item Graph pretraining \& existing work for molecuelar domain 
%     \item Overview \& contribution of this work
% \end{itemize}

% Pretraining has achieved success on a variety of applications, text (NLP), image, etc. Pretraining is to learn representation 
% The advantage of pretraining is one can learn useful representation by leveraging on a large amount of pretraining data. In order to a useful prepresentation that can benefit downstream tasks, different pretraining tasks 




%Graph pretraining is to perform pretraining to utilize graph structure, such as vertex and edges. For example, masking pretraining. masking node and predict the node label, masking edge to predict edge label. Context prediction: 



%However, we investigate several pretraining tasks and the performance compared with downstream task without pretraining to evaluate different performance of downstream tasks.  tested a few


%pretraining and downstream supervision has different objectives. 

% 0 Introduction 
% 1 experiment details 
%     comments / conclusion 
% 2 summery of conclusion/ take away 
% 3 analysis hypothesis 
% 4 limitations 

%The design of pretraining task is 

%A large variety of pretraining methods for molecular application have been proposed, including unsupervised pretraining, supervised pretraining, contrastive learning. However, the effectiveness of these methods remains unclear. The authors found to reproduce some of the reported large gain of graph pretraining results are non-trivial, if not unlikely. The good performance of downstream is largely relied on extensive hyper parameters tuning, which alarms us to rethink how effectiveness self-supervised graph pretraining is and what influence the effectiveness of graph pretraining. All these motivate this paper. 

%The main goal of this study was therefore to compare the performance of proposed graph pretraining methods and 


%Grover \citep{rong2020self}

%ICLR \citep{hu2019strategies}

 
%ICLR requires electronic submissions, processed by
%\url{https://openreview.net/}. See ICLR's website for more instructions.

%If your paper is ultimately accepted, the statement {\tt
%  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
%format to the camera ready requirements.

%The format for the submissions is a variant of the NeurIPS format.
%Please read carefully the instructions below, and follow them
%faithfully.

%\section{Overview: Investigate performance of pretraining on downstream tasks}
%We investigate the following aspects that may influence the performance of pretraining on downstream tasks. We summarize in the following overview. 

% \begin{itemize}
%     \item[$\circ$] Pretraining objectives 
%     \begin{itemize}
%         \item Masking 
%             \begin{itemize}
%                 \item[-] Node
%                 \item Context 
%              \end{itemize}
%         \item[$\circ$]  Contrastive 
%             \begin{itemize}
%                 \item Augmentations 
%                 \item Reaction
%             \end{itemize}
%         \item[$\circ$] Graph-level supervision
%     \end{itemize}
%     \item Split
%     \item Feature
%     \item Architecture
%     \item Data scale
    
    
% \end{itemize}

 


% \begin{enumerate}
%     \item Pretraining objectives 
%         \begin{enumerate}
%             \item Masking 
%                 \begin{enumerate}
%                     \item Node
%                     \item Context 
%                 \end{enumerate}
%             \item  Contrastive 
%                 \begin{enumerate}
%                     \item Augmentations 
%                     \item Reaction
%                 \end{enumerate}
%             \item Graph-level supervision
%                 \begin{enumerate}
%                     \item Supervosed learning
%                 \end{enumerate}
        
%         \end{enumerate}
%     \item Split
%         \begin{enumerate}
%             %\item Uniform
%             \item Balanced scaffold 
%             \item Scaffold 
%         \end{enumerate}
    
%     \item Feature
%         \begin{enumerate}
%             \item Basic feature
%             \item Rich feature 
%         \end{enumerate}
%     \item Architecture
%         \begin{enumerate}
%             \item GIN
%             \item Graph transformer
%             \item graphsage
%         \end{enumerate}
%     \item Data scale
    
%         \begin{enumerate}
%             \item 2M 
%             \item SAVI (1,063,045,046)
%         \end{enumerate}
    
    
% \end{enumerate}




==> [NeurIPS2022-axive]Does GNN Pretraining Help Molecular Representation_/limitation.tex <==
%\vspace{-3mm}
\section{Limitations of current study}
\label{sec:limitation}
%\vspace{-3mm}
Although we have tried our best to design a comprehensive study on the effectiveness of graph pretraining for molecular representation, there are still limitations we want to point out. Due to the limited time and resources we have, we are not able to fully cover the whole picture of the current pretraining paradigm in graph neural networks. Nevertheless, we list them here in hope of preventing the over-generalization of our conclusion.
\begin{itemize}[leftmargin=*,nosep]
    \item \textit{Distribution of graphs}. Our study focuses on pretraining for small molecule graph inductive representation learning. Recently there are works on pretraining transductive representation learning~\citep{you2020does} on large graphs~\citep{hu2020gpt}, where our conclusion may not be directly extended to these cases. 
    \item \textit{Graph architectures}. GNN is a popular research field where many new architectures with probable expressiveness are/will be proposed. The results we have shown are on two representative 1-WL GNNs. It can be possible that the latest advances of deep GNN~\citep{liu2020towards} and Transformer-based GNN~\citep{ying2021transformers, chen2022structure, kim2022pure} might yield different results.
    \item \textit{Learning objectives}. Although we have presented results with different types of self-supervised losses, there are still many variants of each type that we did not explore, like different variants~\citep{sun2021mocl, xia2022simgrace} of contrastive learning. Also, multi-task learning of different self-supervised objectives might be another direction for further exploration.
    \item \textit{Downstream datasets}. We obtained our conclusion mainly on the datasets from MoleculeNet~\citep{wu2018moleculenet}. Datasets like Alchemy~\citep{chen2019alchemy} and drug-target Interaction~\citep{liu2021pre} may show different results.
\end{itemize}


==> [NeurIPS2022-axive]Does GNN Pretraining Help Molecular Representation_/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
% \newcommand{\figleft}{{\em (Left)}}
% \newcommand{\figcenter}{{\em (Center)}}
% \newcommand{\figright}{{\em (Right)}}
% \newcommand{\figtop}{{\em (Top)}}
% \newcommand{\figbottom}{{\em (Bottom)}}
% \newcommand{\captiona}{{\em (a)}}
% \newcommand{\captionb}{{\em (b)}}
% \newcommand{\captionc}{{\em (c)}}
% \newcommand{\captiond}{{\em (d)}}


% Highlight a newly defined term
%\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
%\def\secref#1{section~\ref{#1}}
\def\secref#1{Section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
% \newcommand{\train}{\mathcal{D}}
% \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
%\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
%\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
 
 % The true underlying data generating distribution
% \newcommand{\pdata}{p_{\rm{data}}}
% % The empirical distribution defined by the training set
% \newcommand{\ptrain}{\hat{p}_{\rm{data}}}
% \newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% % The model distribution
% \newcommand{\pmodel}{p_{\rm{model}}}
% \newcommand{\Pmodel}{P_{\rm{model}}}
% \newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% % Stochastic autoencoder distributions
% \newcommand{\pencode}{p_{\rm{encoder}}}
% \newcommand{\pdecode}{p_{\rm{decoder}}}
% \newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
% \newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\emp}{\tilde{p}}
% \newcommand{\lr}{\alpha}
% \newcommand{\reg}{\lambda}
% \newcommand{\rect}{\mathrm{rectifier}}
% \newcommand{\softmax}{\mathrm{softmax}}
% \newcommand{\sigmoid}{\sigma}
% \newcommand{\softplus}{\zeta}
% \newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
% \newcommand{\standarderror}{\mathrm{SE}}
% \newcommand{\Cov}{\mathrm{Cov}}
% % Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% % But then they seem to use $L^2$ for vectors throughout the site, and so does
% % wikipedia.
% \newcommand{\normlzero}{L^0}
% \newcommand{\normlone}{L^1}
% \newcommand{\normltwo}{L^2}
% \newcommand{\normlp}{L^p}
% \newcommand{\normmax}{L^\infty}

% \newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
% \let\ab\allowbreak

% % customer 
% \newcommand{\rbr}[1]{\left(#1\right)}
% %\newcommand{\chapref}[1]{Chapter~\ref{#1}}
%\newcommand{\secref}[1]{Section~\ref{#1}}
% %\newcommand{\secref}[1]{Sec~\ref{#1}}
% \newcommand{\eqnref}[1]{Eq~(\ref{#1})}
% \newcommand{\eqnsref}[1]{Eqns~(\ref{#1})}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
% %\newcommand{\algref}[1]{Algorithm~\ref{#1}}
% \newcommand{\lemref}[1]{Lemma~\ref{#1}}
% \newcommand{\propref}[1]{Proposition~\ref{#1}}
% \newcommand{\thmref}[1]{Theorem~\ref{#1}}
% \newcommand{\asmpref}[1]{Assumption~\ref{#1}}
%\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
% \newcommand{\corref}[1]{Corollary~\ref{#1}}
% %\renewcommand{\algorithmiccomment}[1]{\bgroup\hfill//~#1\egroup}

% \newcommand{\ea}{\emph{et al.}}
% \newcommand{\eg}{\emph{e.g.}}
% \newcommand{\ie}{\emph{i.e.}}
% \newcommand{\iid}{\emph{i.i.d.}}
% \newcommand{\etc}{\emph{etc.}}

% %\newcommand{\rbr}[1]{\left(#1\right)}
% \newcommand{\sbr}[1]{\left[#1\right]}
% \newcommand{\cbr}[1]{\left\{#1\right\}}

% \newcommand{\EE}{\mathbb{E}} % Expectation

% \newcommand{\II}{\mathbb{I}} % Indicator
% \newcommand{\Pscr}{\mathscr{P}}
% \newcommand{\RR}{\mathbb{R}} % Real numbers
% \newcommand{\Xcal}{\mathcal{X}}
% %\newcommand{\Tcalb}{\bm{\Tcal}}
% \newcommand{\Tcal}{{\mathcal{T}}}



==> [NeurIPS2022-axive]Does GNN Pretraining Help Molecular Representation_/results.tex <==
%\vspace{-3mm}
\section{Results}
\label{sec:results}
%\vspace{-3mm}
In this section, we present the results and discussions for a set of experiments designed with the protocols in \Secref{sec:protocol}. \tabref{tab:summary-table} summarizes the experimental configurations for each following table. We will elaborate on them in the following sections. 
Due to space limit, we defer our investigation on different GNN architectures to appendix (\secref{sec：gnn}).

%\input{summary_table}
%\vspace{-2mm}
\subsection{Vanilla configuration}
%\vspace{-1mm}
We choose the \emph{vanilla configuration} with the settings from existing works~\citep{hu2019strategies, rong2020self}. Specifically, we use the \textbf{rich feature} with \textbf{GIN} backbone, pretrained on \textbf{ZINC15} when pretraining is applied, and evaluate on the \textbf{Balanced Scaffold Split} for downstream tasks. One important baseline is without pretraining. For the ease of comparison, we include the results without pretraining in each table.
%\vspace{-2mm}
\subsection{Self-supervised pretraining objectives}
We compare the results pretrained with different self-supervised pretraining objectives. As is presented in \Secref{sec:design_choice}, we consider four representative types of pretraining objectives. For the ease of comparing the performance, we only consider one objective at a time, instead of mixing different pretraining objectives to obtain a multi-task pretrained model. 
\tabref{tab:unsupervised-obj} shows the performance on downstream molecule property prediction benchmarks with models initialized from different pretraining objectives. The relative average gain compared to the one without pretraining is not statistically significant, i.e., not larger than the standard deviations of multiple runs. All the four different objectives obtain similar gains/loses regardless of very different designs. To fully understand the effect of self-supervised pretraining on molecule representation, we further investigate the performance of different pretraining objectives in combination with other factors, such as input features or data splits, as described in the following sections. 
%\vspace{-2mm}
\subsection{Supervised pretraining objectives}
In addition to the self-supervised objectives, we study the potential benefits with supervised pretraining. Unlike the self-supervised setting where the molecule graphs themselves are used for pretraining, the supervised pretraining requires extra cost of data labeling, and thus is not scalable for large scale pretraining. In this paper, we present the results with supervised pretraining alone, as well as the joint pretraining. e.g. pretrain with self-supervised objective and followed by supervised pretraining, in \tabref{tab:super-obj}. We can see with the supervised pretraining, one can improve the downstream performance, which aligns with the observation from \citet{hu2019strategies}. Our hypothesis is that, supervised pretraining is helpful when the pretraining tasks are closely aligned with the downstream tasks. In particular, the bio-activity labels provided by ChEMBL is highly related to the drug discovery purpose and drug discovery properties are the major topics evaluated in the downstream tasks. %\tabref{tab:super-obj} shows that the downstream tasks that are directly measuring biophysical property for drug discovery, such as toxicity, obtain the largest performance improvement from ChEMBL pretraining (e.g. TOXCAST and TOX21). %On the contrary, tasks that do not directly measure drug-able property such as BBBP (predict blood-brain barrier) achieve less gain.  
Therefore, the positive correlation between the pretraining supervision and downstream tasks contribute the most to the performance improvement of downstream tasks. %Based on this fact, the requirement for additional labels and the close alignment between pretraining and downstream tasks can limite the useage of supervised pretraining. 
%\vspace{-3mm}
\subsection{Data split on downstream tasks}
Molecular data is usually diverse and limited, so chemists are particularly interested in the generalization ability of GNNs on out of distribution data. Also due to the same reason (i.e. limited and diverse data), the variance in performance of different splits is significant, which poses challenges on robust evaluation. In \emph{vanilla configuration} we use the balanced scaffold split, and here we show additional results with the \textbf{scaffold} split, which is a deterministic data split that makes the train/valid/test set differ from each other the most.  \tabref{tab:split} and \tabref{tab:feature-scaffold-richfeature-supervised} respectively present the results using scaffold split with self-supervised without and with additional supervised pretraining. Compared with \tabref{tab:unsupervised-obj} and \tabref{tab:super-obj}, it is clear to see that \tabref{tab:split} and \tabref{tab:feature-scaffold-richfeature-supervised} have significantly lower ROC-AUC. Specifically the AUC drops 6.2\% on average for all benchmarks without pretraining. On the other hand, we can see if we compare \tabref{tab:split} with \tabref{tab:unsupervised-obj}, or \tabref{tab:feature-scaffold-richfeature-supervised} with \tabref{tab:super-obj} respectively, the gain of pretraining is more significant on the \textbf{scaffold} split. We 
speculate the reason for the improvement of scaffold split is that the initialization of neural network parameters (e.g. from pretraining) are typically critical for the out-of-distribution generalization (e.g. scaffold split). Similar observations have also been studied in the meta-learning literature~\citep{finn2017model}.  Although the gain with supervised pretraining is significant in \tabref{tab:feature-scaffold-richfeature-supervised},  the effect of self-supervised pretraining is mixed in \tabref{tab:split}. This indicates the effectiveness of self-supervised pretraining on scaffold split is not significant enough to claim ``very helpful''.  
%\vspace{-3mm}
\subsection{Graph features}
%\vspace{-2mm}
So far we have presented the results with rich features. Now we want to see how those basic features used in~\citet{hu2019strategies} affect the outcome. \tabref{tab:Balanced scaffold + basic feature + unsupervised} and \tabref{tab:Balanced scaffold + basic feature + supervised} show the test ROC-AUC (\%) performance with {\it basic features} on the balanced scaffold splits using self-supervised or supervised pretraining objectives, respectively. \tabref{tab:Scaffold + basic feature + unsupervised} and \tabref{tab:Scaffold + basic feature +  supervised} show the same results but on scaffold split. %instead. 

In a nutshell, without pretraining, rich features lead to an average gain of $1.3\%$ and $3.1\%$ over basic features using balanced scaffold split and scaffold split, respectively. Specifically, it achieves $76.7\%$ vs $78.0\%$ for balanced scaffold split, and $68.7\%$ vs $71.8\%$ on scaffold split. The gain brought by the rich features are more significant than the ones with different self-supervised pretraining objectives. \tabref{tab:Balanced scaffold + basic feature + unsupervised} to \tabref{tab:Scaffold + basic feature +  supervised} show that pretraining has more positive impact when basic features are used. In particular, the self-pretraining with context prediction shows significant gains especially in the {scaffold split} setting. However, the gain diminishes when careful feature engineering are applied to the downstream tasks (use rich feature in \emph{vanilla configuration}). The supervised pretraining continues the significant gain under these settings, which shows the consistency and reliability of the situation with the labeled and downstream-task-aligned supervisions. %Specifically, the gain brought by supervised pretraining can be more significant than the rich feature engineering alone. 
%\vspace{-7.5mm}
\subsection{Pretraining datasets}
\label{sec:exp_data_size}
%\vspace{-2mm}
\begin{table*}[t]
\centering
%\vspace{-5mm}
\caption{\textbf{Large scale pretraining data} with balanced scaffold split. No pretraining gets an average AUC of 78.0\%. \label{tab:savi-balanced-split}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllr}
%\hline
\Xhline{2\arrayrulewidth}
Methods        & \textbf{BBBP}  & \textbf{BACE}  & \textbf{TOX21} & \textbf{TOXCAST} & \textbf{SIDER}   & \textbf{AVE GAIN}\\ 
%\hline
\Xhline{2\arrayrulewidth}
\nopretrain      & 92.23($\pm$3.07) & 87.43($\pm$1.63)     & 79.2($\pm$1.99)  & 69.13($\pm$0.55) & 61.92($\pm$0.89) & 0($\pm$1.626)\\
\masktask     & 92.33($\pm$2.08) & 87.22($\pm$1.79) & 79.12($\pm$1.62) & 69.47($\pm$0.65)   & 61.24($\pm$1.94)  &  -0.106($\pm$1.616)  \\
\contexttask  &  93.32($\pm$0.53) & 87.77($\pm$2.94) & 79.18($\pm$2.48) & 70.13($\pm$0.56) & 62.24($\pm$2.65)  &  0.546($\pm$1.832) \\ 
\Xhline{2\arrayrulewidth}
\rowcolor{Gray}
\supervisedmasktask     & 93.23($\pm$3.02) & 86.39($\pm$1.67) & 81.89($\pm$1.58) & 71.77($\pm$0.50)  & 63.73($\pm$2.20)   &  1.420($\pm$1.794) \\
\rowcolor{Gray}
\supervisedcontexttask & 92.55($\pm$2.93) & 87.76($\pm$1.87) & 82.19($\pm$1.58) & 72.91($\pm$0.71) & 62.44($\pm$0.45)  &  1.588($\pm$1.508) \\
%\hline
\Xhline{2\arrayrulewidth}
 %\vspace{-10mm}
\end{tabular}%
}
\end{table*}


\begin{table*}[t]
% \small
\caption{\textbf{Large scale pretraining} data with scaffold split. No pretraining gets an average AUC of 71.8\%. \label{tab:SAVI-scaffold-split}}
%\vspace{-3mm}
\vspace{2mm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllr}
%\hline
\Xhline{2\arrayrulewidth}
Methods               & \textbf{BBBP}  & \textbf{BACE} & \textbf{TOX21} & \textbf{TOXCAST} & \textbf{SIDER}  &  \textbf{AVE GAIN}\\ 
%\hline
\Xhline{2\arrayrulewidth}
\nopretrain             & 74.83($\pm$0.73) & 80.10($\pm$0.42) & 75.86($\pm$0.58)  & 65.95($\pm$0.15) & 62.30($\pm$1.14)  & 0($\pm$0.604)\\
\masktask               & 73.81($\pm$1.82) & 81.90($\pm$1.59) & 74.94($\pm$0.05) & 66.95($\pm$0.12)  & 62.93($\pm$0.34)  &  0.298($\pm$0.784) \\
\contexttask            & 74.32($\pm$0.85) & 83.93($\pm$0.24) & 74.42($\pm$0.19) & 67.01($\pm$0.29)  & 64.83($\pm$0.45)  & 1.094($\pm$0.404)\\ 
\Xhline{2\arrayrulewidth}
\rowcolor{Gray}
\supervisedmasktask     & 73.32($\pm$0.60) & 83.38($\pm$1.05) & 78.59($\pm$0.09) & 67.01($\pm$0.18)  & 65.40($\pm$0.12)  & 1.732($\pm$0.408)\\
\rowcolor{Gray}
\supervisedcontexttask  & 74.38($\pm$0.93) & 86.33($\pm$0.16) & 78.16($\pm$0.25) & 68.71($\pm$0.07)  & 62.22($\pm$0.48)  & 2.152($\pm$0.378)\\
%\hline
\Xhline{2\arrayrulewidth}
%\vspace{-10mm}
\end{tabular}%
}
\end{table*}

As observed in natural language processing domain, more text pretraining data lead to better downstream performance. Intuitively this can be true for molecule representation domain as well, so we run a new set of experiments with the model pretrained on SAVI dataset, which is about 500 times larger than the ZINC15 dataset we used in the above result sections. We present the results pretrained on SAVI dataset using balanced scaffold split or scaffold split in \tabref{tab:savi-balanced-split} and \tabref{tab:SAVI-scaffold-split}, respectively. Other configurations are the same as the \emph{vanilla configuration}. 

Compared with the performance on ZINC15, the SAVI pretraining data does not lead to a significant improvement either on balanced scaffold split  (\tabref{tab:unsupervised-obj} vs \tabref{tab:savi-balanced-split}) or scaffold split (\tabref{tab:split} or \tabref{tab:SAVI-scaffold-split}). Similarly, the self-supervised pretraining objectives lead to negligible gain on downstream task performance, while the supervised one still achieves a clear gain. 

As the result is counterintuitive, we further investigate the reason behind it by inspecting the pretraining performances with different training objectives on both ZINC15 and SAVI datasets. We plot the curve of accuracy growth with the number of training steps iterated. We can see from \Figref{fig:pretraining} that in all settings the pretraining accuracy grows above 90\% quickly after only 0.1 to 0.2M steps and also converges quickly. Given that the model gets very high accuracy without even going through 1 epoch of the SAVI dataset, it is expected that the larger training data like SAVI may not provide more learning signals for the model, and partially explains why more molecules wouldn't help significantly in this case. Furthermore, these figures might suggest several reasons of why the self-supervised pretraining may not be very effective in some situations:
\begin{itemize}[noitemsep,topsep=2pt,parsep=6pt,partopsep=2pt, leftmargin=*]
	\item \textbf{Tasks are easy.} Some of the self-pretraining tasks for molecules might be easy, so that model learns less useful information from pretraining. For example in the masked node prediction case, the model is expected to predict the atomic number from a vocabulary with less than 100 candidate atoms. Furthermore, due to the valence constraints, the graph topology may already exclude most of the wrong atoms. As a comparison, the vocabulary size for text pretraining may be 100k or even higher. Some structured prediction tasks like context prediction might be hard, but due to the difficulty of structured prediction itself and the proposal for high quality negative examples for contrastive learning, it can still be challenging for downstream task improvements. Other strategies like motif prediction can be achieved by subgraph matching, which can be easy for GNN that intrinsically does the graph isomorphism test.
	\item \textbf{Data lacks diversity.} Due to biophysical and functional requirements, molecules share many common sub-structures, e.g., functional motifs. Hence, molecules may not be as diversified as text data. This is why the model learns to generalize quickly within the training distribution. 
	\item \textbf{2D Structure is not enough to infer functionality.} Some important biophysical properties (such as 3D structure, chirality) are barely reflected in the 2D-feature-based pretraining (e.g., using smiles or 2D graph features). For example, the molecules with the same chemical formula and 2D feature, can have very different chirality, which leads to quite different toxicity \citep{smith2009chiral} (e.g. flipped toxicity labels). This is not captured in the current GNN pretraining frameworks that we considered.
\end{itemize}
%\vspace{-1mm}


%\begin{wrapfigure}{r}{0.5\textwidth}
%\begin{figure}%[t]
%\centering
%\includegraphics[width=0.46\textwidth]{figs/pretrain-4.pdf}
%\caption{Pretraining accuracy on ZINC15 or SAVI datasets with node prediction or context prediction objectives. \label{fig:pretraining}}
%\vspace{-1mm}
%\end{figure}
%\end{wrapfigure}


\begin{wrapfigure}{r}{0.59\textwidth}
 \vspace{-9mm}
  \begin{center}
    \includegraphics[width=0.36\textwidth]{figs/pretrain-4.pdf}
  \end{center}
  \vspace{-3mm}
 \caption{Pretraining accuracy on ZINC15 or SAVI datasets with node prediction or context prediction objectives. \label{fig:pretraining}}
 \vspace{-3mm}
\end{wrapfigure}
%\subsection{GNN architecture} 
%We also investigate GNN
% \vspace{-4mm}
\subsection{Hyper-parameters for downstream tasks}
We also find that hyper-parameters for downstream tasks are critical for the their performance that their choices may change the conclusion of the effectiveness of pretraining in some settings.
% For example, learning rate is important. 
We can take the learning rate as an example.
As the models initialized from scratch and pretraining may have different scales, the most suitable learning rate required for downstream tasks may also be different. Without tuning learning rate extensively, we may reach a misleading conclusion.
In particular, when we adopt the default learning rate for reproducing the existing success of pretraining in \tabref{tab:feature-balancedscaffold-basicfeature-wrong} of Appendix~\ref{sec:reproduce}, we indeed observe the advantage of pretraining. However, if we follow our procedures (e.g. extensive search learning rate and averaging over three splits), the resulting \tabref{tab:unsupervised-obj} and \tabref{tab:super-obj} indicate no performance gain by pretraining. So we suggest that the evaluation of pretraining should consider the hyper-parameter tuning and averaging over different splits. 







==> [NeurIPS2022-axive]Does GNN Pretraining Help Molecular Representation_/summary.tex <==
%\vspace{-1mm}
\section{Summary and takeaways}
\label{sec:summary}
%\vspace{-1mm}
Based on our experiments in \secref{sec:results}, we present our takeaways by empirically summarizing our conjectures on when the pretraining would/would not help the molecular representation learning.
%\vspace{-3mm}
\paragraph{When pretraining might help} We find it typically helps 1) if we can have the supervised pretraining with target labels that are aligned with the downstream tasks. However, getting large amount of high-quality and relevant supervision is not always feasible; 2) if the high quality hand-crafted features are absent. However, it seems that the gain obtained by self-supervised pretraining is not as significant as these high quality hand-crafted features based on our current studies; 3) if the downstream train, valid and test dataset distributions are substantially different.
%\vspace{-3mm}
\paragraph{When the gain diminishes?} In some situations the gain of pretraining might diminish 1) if we already have the high quality hand-crafted features (e.g. rich features described in \secref{sec:design_choice}); 2) if we don't have the highly relevant supervisions. As shown in \secref{sec:exp_data_size}, many self-supervised pretraining tasks might be too easy for the model to learn meaningful embedding; 3) if the downstream data splits are balanced; 4) if the self-supervised learning dataset lacks diversity, despite its scale.
\paragraph{Why pretraining may not help in some cases?} In our paper we pretrained a GNN on a much larger dataset (SAVI) than before, hoping to replicate gain of pretraining like in NLP domain. However, we do not obtain the expected gain. The pretraining accuracy curve (\Figref{fig:pretraining}) provides some potential explanations of why pretraining may not work: some of the pretraining accuracy curve grows above $95\%$+ quickly and converges fast, unlike pretraining in NLP which keeps growing to $70\%$ and hardly plateaus. This suggests that some of the pretraining methods like masked node label prediction might be easy (as the vocabulary size is much smaller compared to NLP) and therefore transfer less knowledge for downstream tasks.


==> [NeurIPS2022-axive]Does GNN Pretraining Help Molecular Representation_/summary_table.tex <==
\begin{table*}[th]
\centering
%\vspace{-5mm}
\caption{Summary of Experiments. \tabref{tab:graphsage + neurips split} and \tabref{tab:graphsage + iclr split} are deferred to appendix due to space limit. \label{tab:summary-table}}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{c|cc|cc|cc|cc|cc}
%\hline
\Xhline{2\arrayrulewidth}
 &
  \multicolumn{2}{c|}{\textbf{Pretrain Objective}} &
  \multicolumn{2}{c|}{\textbf{Graph Features}} &
  \multicolumn{2}{c|}{\textbf{Downstream Splits}} &
  \multicolumn{2}{c|}{\textbf{GNN Arch}} &
  \multicolumn{2}{c}{\textbf{Pretrain Dataset}} \\ 
  \cline{2-11}
  %\xchline{2-11}{2\arrayrulewidth}
 &
{Self-Supervised} &
{Supervised} &
{Rich} &
{Basic} &
{Balanced} &
{Scaffold} &
{GIN} &
{GraphSage} &
{ZINC15} &
{SAVI} \\
  %\hline
  \Xhline{2\arrayrulewidth}
\textbf{\tabref{tab:unsupervised-obj}} 
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:super-obj}} 
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:split}} 
   &\ding{52}
   &
   &\ding{52}
   &
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:feature-scaffold-richfeature-supervised}} 
   &
   &\ding{52}
   &\ding{52}
   &
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:Balanced scaffold + basic feature + unsupervised}} 
   &\ding{52}
   &
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:Balanced scaffold + basic feature + supervised}}
   &
   &\ding{52}
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:Scaffold + basic feature + unsupervised} }
   &\ding{52}
   &
   &
   &\ding{52}
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:Scaffold + basic feature + supervised}}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
%\textbf{\tabref{tab:graphsage + neurips split}} 
%   &\ding{52}
%   &\ding{52}
%   &\ding{52}
%   &
%   &\ding{52}
%   &
%   &
%   &\ding{52}
%   &\ding{52}
%   &
%   \\ \hdashline
%\textbf{\tabref{tab:graphsage + iclr split}} 
%   &\ding{52}
%   &\ding{52}
%   &\ding{52}
%   &
%   &
%   &\ding{52}
%   &
%   &\ding{52}
%   &\ding{52}
%   &
%   \\\hdashline
\textbf{\tabref{tab:savi-balanced-split}} 
   &\ding{52}
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   & 
   &
   &\ding{52}
   \\\hdashline
\textbf{\tabref{tab:SAVI-scaffold-split}} 
   &\ding{52}
   &\ding{52}
   &\ding{52}
   &
   &
   &\ding{52}
   &\ding{52}
   &
   &
   &\ding{52}
   \\ 
   %\hline
  % \Xhline{2\arrayrulewidth}
  \hdashline 
   \textbf{\tabref{tab:graphsage + neurips split}} 
   &\ding{52}
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   &
   &\ding{52}
   &\ding{52}
   &
   \\ \hdashline
\textbf{\tabref{tab:graphsage + iclr split}} 
   &\ding{52}
   &\ding{52}
   &\ding{52}
   &
   &
   &\ding{52}
   &
   &\ding{52}
   &\ding{52}
   &
   \\\hdashline
     \Xhline{2\arrayrulewidth}
\end{tabular}%
%\vspace{-5mm}
}
\end{table*}



==> [NeurIPS2022] Graph pretraining/abstract.tex <==
\begin{abstract}
%\vspace{-.5em}
Extracting informative representations of molecules using Graph neural networks (GNNs) is crucial in AI-driven drug discovery. Recently, the graph research community has been trying to replicate the success of self-supervised pretraining in natural language processing, with several successes claimed. However, we find the benefit brought by self-supervised pretraining on small molecular data can be negligible in many cases. We conduct thorough ablation studies on the key components of GNN pretraining, including pretraining objectives, data splitting methods, input features, pretraining dataset scales, and GNN architectures, to see how they affect the accuracy of the downstream tasks. Our first important finding is, self-supervised graph pretraining do not always have statistically significant advantages over non-pretraining methods in many settings. Secondly, although noticeable improvement can be observed with additional supervised pretraining, the improvement may diminish with richer features or more balanced data splits. Thirdly, hyper-parameters could have larger impacts on accuracy of downstream tasks than the choice of pretraining tasks, especially when the scales of downstream tasks are small. Finally, we provide our conjectures where the complexity of some pretraining methods on small molecules might be insufficient, followed by empirical evidences on different pretraining datasets.

%\vspace{-1em}
% Therefore, our overall sentiment is different from the previous works that are cheerful on pretraining in thie field, as we do not see clear and unconditional improvements by GNN pretraining yet. 
%All in all, we do not observe clear and unconditional improvements on molecular presentation by GNN pretraining yet,
%thus finally we also provide our empirical investigation on the reasons behind it.

% indicating a lot more efforts are needed in this field to make pretraining a great success.
% Therefore, all these observations motivate us to rethink the effectiveness of graph-pretraining on molecule applications and investigate the underlying reasons.
%} 
 
 
% \adamsyuwei{
% Graph neural networks (GNNs) have proven to be useful modeling tools for molecular data. Recently, 
% people have been trying to replicate the success of pretraining techniques in natural language processing (NLP) to this domain 
% with several success claimed. However, in this paper, our conclusion surprisingly contradicts to those works, as we 
% find the benefit, if any, brought by pretraining a GNN is negligible. We conduct thorough ablation studies on the key components 
% of graph pretraining on molecular data, which include the network architectures, pretraining objective functions, 
% data splitting methods, types of additional features and pretraining dataset sizes. 
% We start with a baseline setting, followed by extensive control experiments on those factors.
% Our finding is, under every single setting, we rarely see the downstream tasks benefit from pretraining. 
% What’s more, the very best pretraining model underperforms the non-pretrained model.
% Further investigation shows that xxxx.
% Our contradictory finding indicates self-supervised pretraining on graph neural network for molecular data has not reached the level of success
% as NLP yet. Hence, a lot more studies are needed before pretraining can take off in this area.
% }

%Graph pretraining is to learn useful representations of graph format data by pretraining on a large amount of data. Those useful representations are applied to benefit downstream tasks. Current graph pretraining has a few categories: masking pretraing, with the goal to benefit downstream tasks. % \mask
\end{abstract}

==> [NeurIPS2022] Graph pretraining/experiment.tex <==
\section{Experiment framework}
\label{sec:exp_framework}
%\vspace{-3mm}
%To design our experimental framework 
%To understand more about the 
To investigate pretraining on graphs for molecule representations, we first revisit the typical pretraining-finetuning pipeline used in the literature. \Figref{fig:pipeline} shows the overall procedure of deployment, with several design choices presented at each stage of the pipeline. Since different choices at each stage can lead to different performances on the downstream tasks, 
we investigate them one at a time while keeping others the unchanged. %
The design principle of our experiment framework is to analyze the effect of \emph{every} stage in the pipeline as comprehensive as possible, while also keeping it tractable to avoid exponentially many experiments. %Below we describe these stages and the corresponding design choices we considered in the experiments. 
%\vspace{-3mm}
\subsection{Design choices}
\label{sec:design_choice}
%\vspace{-4mm}
We consider the design choices for the four pretraining objectives.
%\vspace{-1mm}
\paragraph{Pretraining objective} In \Secref{sec:gnn_pretrain} we have provided a brief literature review over the pretraining methods for molecule representation. Here we categorize those pretraining by different principles, and present one well-recognized representative of each category. The representatives are selected because they have more desired properties, such as better performance, compared with their counterparts. 
\begin{itemize}[noitemsep,topsep=3pt,parsep=3pt,partopsep=5pt, leftmargin=*]
	\item \textbf{Masking.} We leverage the node prediction objective, which randomly masks 15\% of the nodes' feature and then ask GNN to make prediction on the node attributes of the masked ones. This strategy %is %from~\citet{hu2019strategies} and 
	resembles the BERT pretraining~\citep{devlin2018bert} in natural language processing.
	\item \textbf{Structured.} Unlike text data where the topology is a sequence, the graph has rich structure information. Following~\citet{hu2019strategies}, we use context prediction objective, which masks out the context from $k_1$-hops to $k_2$-hops and leverages  adversarial training to predict the true context embeddings from the random context embeddings. 
	\item \textbf{Graph-level self-supervised.} Following \citep{rong2020self}, GNN is asked to predict whether a motif is contained in a molecule. The motif can be extracted from the molecule with RDKit~\citep{landrum2016rdkit}. %We denote it as \textbf{Motif Prediction}, and use the same set 
The motifs are 85 motifs~\footnote{\url{http://rdkit.org/docs/source/rdkit.Chem.Fragments.html}} %as~\citep{rong2020self}
	for multi-label classification. 
	\item \textbf{Contrastive.}  We generate two views of the same graph by corrupting the input node features with Gaussian noise. %to generate different views of the same graph, %and leverage the locally normalized probability to
	We leverage the contrastive learning loss proposed in ~\citep{you2020graph}: we maximize the consistency between positive pairs (from same graphs) and minimize that between negative pairs (from different graphs). In this paper, we restrict ourselves to this specific contrastive training method, however, various contrastive learning methods can be further explored. 
	\item \textbf{Graph-level supervised.} Finally when applicable, we use the ChEMBL dataset with graph-level labels for graph-level supervised pretraining as ~\citet{hu2019strategies}. 
\end{itemize}

The above are the design choices for pretraining objectives. %In addition to these stages, we believe the factors in downstream applications can potentially affect the effectiveness of pretraining as well. 
Next, we consider other factors that influence graph-pretraining performance. %the configurations for the finetuning stages in the downstream tasks. 
%\vspace{-4mm}
%\paragraph{Learning hyperparameters for downstream tasks} We find that the models initialized from pretrained checkpoints and those from scratch may favor different hyperparameter configurations like learning rates. So to make a fair comparison, we would tune the learning rate separately for each setting, instead of using the same configuration for all the settings. This is critical for the fair comparison of performance on downstream tasks. 
%\vspace{-4mm}
\paragraph{Graph Features} Each molecule is represented by a graph with atoms as nodes and bonds as edges. In this paper we mainly consider the graph representations without the 3D information. %Generally speaking, in each of such a graph, each node (atom) or edge (bond) is associated with a binary feature vector. The features are constructed based on domain knowledge, and 
%The features prepared for graph neural networks are 
For each molecule graph, chemical properties of nodes and edges are extracted to serve as node and edge features for the graph neural networks. Depending on how rich the features are, we categorize the design choices into two categories:
\begin{itemize}[noitemsep,topsep=1pt,parsep=1pt,partopsep=0pt, leftmargin=*]
	\item \textbf{Basic features.} The basic set of features are the ones used in \citet{hu2019strategies}. Specifically, the node features contain the atom type and the derived features, such as formal charge list, chirality list, etc. The edge features contain the bond types and the bond directions. These features are categorical, and thus will be encoded in a one-hot vector individually and then concatenated together to form the feature vector for node/edge representation. 
	\item \textbf{Rich features.} The rich feature set is a superset of the basic features. In addition to the basic ones mentioned above, it comes with the additional node features such as hydrogen acceptor match, acidic match and bond features such as ring information. This set of features are used in ~\citet{rong2020self}. Additionally and importantly, we follow their setting to incorporate additional 2d normalized rdNormalizedDescriptors features~\footnote{ \url{https://github.com/bp-kelley/descriptastorus} for the feature descriptor.}, which is used in the downstream tasks only and not in pretraining.
\end{itemize}
Please refer to the original papers for the full set of basic~\citep{hu2019strategies} and rich~\citep{rong2020self} features, respectively.

\begin{table*}[t]
\small
%\vspace{-3mm}
\centering
\caption{Self-supervised + \textbf{Basic feature} + Balanced Scaffold. No pretrain has an average AUC of 76.7\% over all 5 datasets. \label{tab:Balanced scaffold + basic feature + unsupervised}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
%\hline
\Xhline{2\arrayrulewidth}
Methods                   & \textbf{BBBP}                           & \textbf{BACE}                           & \textbf{TOX21}                          & \textbf{TOXCAST}                        & \textbf{SIDER}        &    \textbf{AVE GAIN}                    \\ 
%\hline
\Xhline{2\arrayrulewidth}
\nopretrain              & 91.46($\pm$ 0.85) &  84.29($\pm$ 3.80) &  78.35($\pm$ 0.95)  & 68.31($\pm$ 1.61) & 61.15($\pm$ 2.46)  &  0($\pm$1.934)\\
\masktask                & 91.23($\pm$ 1.51) & 84.97($\pm$ 1.55) & 77.77($\pm$ 1.23) & 68.98($\pm$ 1.11) & 61.20($\pm$ 0.41)  &   0.118($\pm$1.162)\\
\contexttask             & 92.13($\pm$ 1.04) & 84.83($\pm$ 3.19) & 78.79($\pm$ 2.52) & 68.29($\pm$ 1.23) & 62.32($\pm$ 2.99) &   0.560($\pm$2.194)\\
%\supervisedtask              & 90.70($\pm$ 0.74)  & 84.22($\pm$ 2.69) & 80.45($\pm$ 1.47) & 69.47($\pm$ 1.06) & 63.38($\pm$ 1.44) \\
%\supervisedmasktask     & 91.10($\pm$ 2.88)  & 85.54($\pm$ 4.57) & 81.49($\pm$ 1.52) & 70.77($\pm$ 1.00)  & 62.81($\pm$ 2.61) \\
%\supervisedcontexttask & 91.54($\pm$ 3.52) & 85.71($\pm$ 2.92) & 81.23($\pm$ 1.94) & 71.36($\pm$ 1.05) & 62.75($\pm$ 2.27) \\ 
%\hline
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\end{table*}


\begin{table*}[t]
% \small
%\vspace{-4mm}
\centering
\caption{Supervised + %Self-supervised +
\textbf{Basic feature} + Balanced Scaffold. No pretrain has an average AUC of 76.7\%. \label{tab:Balanced scaffold + basic feature + supervised}}
%\vspace{-3mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
%\hline
\Xhline{2\arrayrulewidth}
Methods                    & \textbf{BBBP}                           & \textbf{BACE}                           & \textbf{TOX21}                          & \textbf{TOXCAST}                        & \textbf{SIDER}     &    \textbf{AVE GAIN}                       \\ 
%\hline
\Xhline{2\arrayrulewidth}
\nopretrain            & 91.46($\pm$ 0.85) &  84.29($\pm$ 3.80) &  78.35($\pm$ 0.95)  & 68.31($\pm$ 1.61) & 61.15($\pm$ 2.46) & 0($\pm$ 1.934) \\
%\masktask                & 91.23($\pm$ 1.51) & 84.97($\pm$ 1.55) & 77.77($\pm$ 1.23) & 68.98($\pm$ 1.11) & 61.20($\pm$ 0.41)  \\
%\contexttask             & 92.13($\pm$ 1.04) & 84.83($\pm$ 3.19) & 78.79($\pm$ 2.52) & 68.29($\pm$ 1.23) & 62.32($\pm$ 2.99) \\
\supervisedtask              & 90.70($\pm$ 0.74)  & 84.22($\pm$ 2.69) & 80.45($\pm$ 1.47) & 69.47($\pm$ 1.06) & \textbf{63.38($\pm$ 1.44)} & 0.932($\pm$ 1.480)\\
\supervisedmasktask     & 91.10($\pm$ 2.88)  & 85.54($\pm$ 4.57) & \textbf{81.49($\pm$ 1.52)} & 70.77($\pm$ 1.00)  & 62.81($\pm$ 2.61) & 1.630($\pm$ 2.516)\\
\supervisedcontexttask & \textbf{91.54($\pm$ 3.52)} & \textbf{85.71($\pm$ 2.92)} & 81.23($\pm$ 1.94) & \textbf{71.36($\pm$ 1.05)} & 62.75($\pm$ 2.27) & 1.806($\pm$ 2.340)\\ 
%\hline
\Xhline{2\arrayrulewidth}
%\vspace{-10mm}
\end{tabular}
}
\end{table*}
%\vspace{-3mm}
\paragraph{GNN Backbone} The GNN architecture also plays a role in graph pretraining. In~\citet{hu2019strategies}, the results show that pretraining on GNN variants like GIN~\citep{xu2018powerful} would improve the performance on downstream tasks, while the performance with architectures like GAT~\citep{velivckovic2017graph} would actually get worse performance with pretraining. As the GNNs based on 1-Weisfeiler-Lehman (WL) test have similar representation power~\citep{xu2018powerful} bounded by the Weisfeiler-Lehman isomorphism check~\citep{shervashidze2011weisfeiler}, we consider the two representative GNN architectures, namely the \textbf{GIN}~\citep{xu2018powerful} and \textbf{GraphSage}~\citep{hamilton2017representation}. They have shown benefits with graph pretraining in ~\citet{hu2019strategies}.
%\vspace{-3mm}
\paragraph{Pretraining dataset} In natural language pretraining, researchers observed a significant performance boost due to self-supervised pretraining on large-scale data, that is, the larger the pretraining dataset is, the better the downstream performance it is ~\citep{raffel2019exploring}. %We hope to obtain similar outstanding performance improvement as a result of pretraining with large scale datasets for graph pretraining. 
Inspired by this success in natural language processing, we test the algorithms on two unlabeled pretraining datasets with different scales.

\begin{itemize}[noitemsep,topsep=1pt,parsep=1pt,partopsep=0pt, leftmargin=*]
	\item \textbf{ZINC15~\citep{sterling2015zinc}}: ZINC15 contains 2 million molecules. This dataset was preprocessed following ~\citet{hu2019strategies}.
	\item \textbf{SAVI ~\citep{patel2020synthetically}}: The SAVI dataset contains about 1 billion molecules, which are significantly larger than ZINC15. To the best of our knowledge, it has never been used for pretraining tasks before. This dataset contains drug-like molecules synthesized by computer simulated reactions. 
	\end{itemize}

Additionaly, we used \textbf{ChEMBL~\citep{gaulton2012chembl}} as the supervised datasets. Different from the above ZINC15 and SAVI dataset which are only used for self-supervised pretraining, this dataset contains 500k drug-able molecules with 1,310 prediction target labels from bio-activity assays for drug discovery. Thus like in~\citet{hu2019strategies} we only leverage it for \emph{supervised} pretraining. 
%\vspace{1mm}
%\vspace{-4.5mm}
% \paragraph{Pretraining objective} In \Secref{sec:gnn_pretrain} we have provided a brief literature review over the pretraining methods for molecule representation learning. Here we categorize these into objectives with different principles, and consider the representative one per each objective categories. 
% \begin{itemize}
% 	\item \textbf{Masking.} We leverage the \textbf{Node Prediction} objective, which randomly mask 15\% of the nodes' features and then ask GNN to make predictions on the node attributes for the masked ones. This strategy is from~\citet{hu2019strategies} and resembles the BERT pretraining~\citep{devlin2018bert} for natural language.
% 	\item \textbf{Structured.} Unlike text data where the topology is a sequence, the graph has rich structure information. Following~\citet{hu2019strategies} we use \textbf{Context Prediction}, which masks out the context from $k_1$-hops to $k_2$-hops and leverages  adversarial training to let the GNN predict the true context embeddings from the random context embeddings. 
% 	\item \textbf{Graph-level self-supervised.} We ask the GNN to predict the motif it contains. The motif can be extracted from the molecule with RDKit~\citep{landrum2016rdkit}. We denote it as \textbf{Motif Prediction}, and use the same set of 85 motifs~\footnote{\url{http://rdkit.org/docs/source/rdkit.Chem.Fragments.html}} as~\citep{rong2020self} for multi-label classification. 
% 	\item \textbf{Contrastive.} We leverage the \textbf{Contrastive Learning} approach in ~\citep{you2020graph} to corrupt the input node features with Gaussian noise, and leverage the locally normalized probability to maximize the consistency between positive pairs and minimize that between negative pairs.
% 	\item \textbf{Graph-level supervised.} Finally when applicable, we use the ChEMBL dataset with graph-level labels for graph-level \textbf{Supervised Pretraining}, as presented in ~\citet{hu2019strategies}. 
% \end{itemize}
% The above four components are the design choices for pretraining stage. In addition to these stages, we believe the factors in downstream applications can potentially affect the effectiveness of pretraining as well. So we also consider the configurations for the finetuning stages in the downstream tasks. 
% \vspace{-2.0 mm}
\paragraph{Data split on downstream tasks} The downstream tasks for molecular domain we used are 5 benchmark datasets from MoleculeNet~\citep{wu2018moleculenet} (See Appendix~\ref{sec:molecular_benchmarks} for more details). The train/valid/test sets are split with ratio 8:1:1. For molecule domain, the random split is not the most meaningful way to assess the performance, because the real-world scenarios often require generalization ability on out-of-distribution samples. So we consider the following ways to split the data:
\begin{itemize}[noitemsep,topsep=1pt,parsep=1pt,partopsep=0pt, leftmargin=*]
	\item \textbf{Scaffold Split~\citep{hu2019strategies, ramsundar2019deep}} This strategy first sorts the molecules according to the scaffold (e.g. molecule structure), and then partition the sorted list into train/valid/test splits consecutively. Therefore, the molecules in train and test sets are most different ones according to their molecule structure.  Note this strategy would yield deterministic data splits.
	\item \textbf{Balanced Scaffold Split~\citep{bemis1996properties, rong2020self}} This strategy introduces the randomness in the sorting and splitting stages above, thus one can run on splits with different random seeds and report the average performance to lower the evaluation variance.
\end{itemize}

We choose balanced scaffold as our major evaluation configuration, because it allows us to evaluate the algorithm on multiple data splits while maintaining the ability to evaluate out of distribution samples (e.g. assess generalization ability). Evaluating on one single split (such as scaffold split) can be subject to bias due to one specific split, leading to higher variance in evaluation. 
%\vspace{-3mm}
%x
\begin{table*}[t]
\small
%\vspace{-3mm}
\centering
\caption{Unsupervised + \textbf{Basic feature + Scaffold}. No pretrain has an average accuracy of 68.7\% over all benckmark datasets. \label{tab:Scaffold + basic feature + unsupervised}}
%\vspace{-3mm}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
\Xhline{2\arrayrulewidth}
%\hline
Methods               & \textbf{BBBP}                & \textbf{BACE}             & \textbf{TOX21}            & \textbf{TOXCAST}              & \textbf{SIDER} &    \textbf{AVE GAIN}    \\ 
%\hline
\Xhline{2\arrayrulewidth}
\nopretrain              & 69.62($\pm$ 1.05)            & 75.77($\pm$4.29)          & 75.52($\pm$0.67)          & 63.67($\pm$0.32)              & 59.07($\pm$1.13)  &   0($\pm$1.492)\\
\masktask                & 68.70($\pm$2.16)             & 76.95($\pm$0.12)          & 75.88($\pm$0.60)          & 64.11($\pm$0.38)              & 61.29($\pm$0.87)  &   0.656($\pm$0.826)\\
\contexttask             & 69.41($\pm$1.44)             & \textbf{81.96}($\pm$0.72)          & 75.49($\pm$0.75)          & 63.48($\pm$0.31)              & \textbf{62.27($\pm$0.90)}  &   1.792($\pm$0.824)\\
%\supervisedtask          & 68.96($\pm$0.64)             & 76.30($\pm$1.30)          & 76.64($\pm$0.39)          & 66.07($\pm$0.22)              & 61.97($\pm$0.96) \\
%\supervisedmasktask      & \textbf{71.41($\pm$0.67)}    & 84.59($\pm$0.35)          & 79.13($\pm$0.29)          & 65.32($\pm$0.37)              & 62.12($\pm$0.19) \\
%\supervisedcontexttask   & 69.63($\pm$0.25)             & \textbf{83.34($\pm$0.67)} & 78.11($\pm$0.28)          & 66.15($\pm$0.48)              & 63.48($\pm$0.43) \\ 
%\hline
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\end{table*}


\begin{table*}[t]
% \small
%\vspace{-5mm}
\centering
\caption{Supervised + \textbf{Basic feature + Scaffold}. No pretrain has an average accuracy of 68.7\% over all benckmark datasets. \label{tab:Scaffold + basic feature + supervised}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
%\hline
\Xhline{2\arrayrulewidth}
Methods                & \textbf{BBBP}                & \textbf{BACE}             & \textbf{TOX21}            & \textbf{TOXCAST}              & \textbf{SIDER}   &    \textbf{AVE GAIN}  \\ 
%\hline
\Xhline{2\arrayrulewidth}
\nopretrain              & 69.62($\pm$ 1.05)            & 75.77($\pm$4.29)          & 75.52($\pm$0.67)          & 63.67($\pm$0.32)              & 59.07($\pm$1.13)   &  0($\pm$1.492)\\
%\masktask                & 68.70($\pm$2.16)             & 76.95($\pm$0.12)          & 75.88($\pm$0.60)          & 64.11($\pm$0.38)              & 61.29($\pm$0.87) \\
%\contexttask             & 69.41($\pm$1.44)             & 81.96($\pm$0.72)          & 75.49($\pm$0.75)          & 63.48($\pm$0.31)              & 62.27($\pm$0.9)  \\
\supervisedtask          & 68.96($\pm$0.64)             & 76.30($\pm$1.30)          & 76.64($\pm$0.39)          & 66.07($\pm$0.22)              & 61.97($\pm$0.96)  &   1.258($\pm$0.702)\\
\supervisedmasktask      & \textbf{71.41($\pm$0.67)}    & 84.59($\pm$0.35)          & \textbf{79.13($\pm$0.29)} & 65.32($\pm$0.37)              & 62.12($\pm$0.19) &    3.784($\pm$0.374)\\
\supervisedcontexttask   & 69.63($\pm$0.25)             & \textbf{83.34($\pm$0.67)} & 78.11($\pm$0.28)          & \textbf{66.15($\pm$0.48)}     & \textbf{63.48($\pm$0.43)} &   3.412($\pm$0.422)\\ 
%\hline
\Xhline{2\arrayrulewidth}
%\vspace{-12mm}
\end{tabular}

}
\end{table*}
\subsection{Experiment protocol}
\label{sec:protocol}
As the total number of configurations for the entire pipeline can be combinatorially large which is not practical for us to exhaustively experiment with all of them, we design our protocol with a pairwise comparison principle. Specifically, we first anchor a \emph{vanilla configuration} with a certain design choice of combination for each stage. To study the effect of each stage on the pretraining effectiveness, we vary the design choice one stage at a time compared to the \emph{vanilla configuration}. %In total we would run $N$ sets of experiments where $N$ is the number of varying stages we considered. Note that in each set of experiments we will still have multiple experiments for each possible design choices we consider for that stage.

%By pairwise comparison between each set of variations and the \emph{vanilla configuration}, we can see how the design choices affect the outcome of the pretraining, and in which scenario will the pretraining help most for the downstream tasks. However, whenever feasible, we can also analyze the effect of joint variations on multiple stages by comparing the results of them together. We will present these results, our analysis and hypothesis in the next section. 

For all these experiments, to assess the effectiveness of graph pretraining, we report the \textbf{ROC-AUC} on downstream tasks as well as the relative \textbf{average gain} over all downstream datasets with and without pretraining. For each setting we will report the mean and standard deviation (in parenthesis) over three runs with different random seeds. We tune the model on downstream tasks with the validation set, and report the evaluation metric on the test set using the model with best validation performance. For each setup, we report the average performance obtained with three random seeds. We tune the learning rate in $\{1e^{-4}, 5e^{-4}, 1e^{-3}, 5e^{-3}, 1e^{-2}, 5e^{-2}, 1e^{-1}\}$ for each setup \emph{individually} and select the one with best validation performance. For GNNs we fix the hidden dimension to 300 and number of layers to 5.

==> [NeurIPS2022] Graph pretraining/gnn_pretrain.tex <==
\section{Preliminary}
\label{sec:gnn_pretrain}

\input{summary_table}

%\section{Graph Pretraining}
%Some data like chemical molecules contains structure information, which can be modeled as a graph. For example, in chemical molecules, atoms are modeled as nodes, and bonds are modeled as edge. Start from some format of node and edge feature, Graph neural networks performs several rounds of convolution of every node using the features of its connected neighbour nodes and the edges between them. After several sounds of convolution, the node feature and edge feature are Therefore, it is a natural way to represent raw format of data into deep-learning usable representation while maintain structure information.  THe representation can be used on pretraining tasks or downstream tasks with different objectives. 
% {\color{red} In graph learning, there
% are usually two categories of supervised tasks: i) Node classification/regression, where each node
% v has a label/target yv, and the task is to learn to predict the labels of unseen nodes; ii) Graph
% classification/regression, where a set of graphs {G1, ..., GN } and their labels/targets {y1, ..., yN } are
% given, and the task is to predict the label/target of a new graph.

% %we divide existing graph SSL methods into three categories: contrastive, generative, and predictive,

% }

%We choose implementation of ICLR paper \citet{hu2019strategies}, as we can reproduce the results reported in the paper, and we can observe gains on the proposed scaffold split under the authors setup. 

\paragraph{Graph Neural Networks (GNNs).} Let $G = \{V, E\}$ denote a molecule graph with $V$ as the set of nodes and $E$ as the set of edges. 
%$X_v$ as node attributes for $v \in V$ and $e_{ij}$ as edge features for edge(i, j) $\in E$. 
Given the node features $X_i$, most GNNs learn an embedding representation $h_i$ for every node $i \in V$ by aggregating representations from connected nodes and edges, denoted as graph convolution. These procedure repeats for $K$ times with the update equation as follows:
\begin{equation}
%\resizebox{1.0\hsize}{!}{$
h_i^k = \text{UPDATE}(h_i^{k-1}, \text{AGGREGATE}(\{h_i^{k-1}, h_j^{k-1}, e_{ij}\}: \forall j \in N(i))) \nonumber
%$}
\end{equation}
where $\gN(i)$ is the set of neighbor nodes of $i$ and $h_i^0 = X_i$. The representation for entire graph $G$ is then obtained by permutation-invariant transformation on node representation,  $h_G = \text{READOUT}(h_i^K | i\in V)$. In this paper we mainly study the GNNs that belong to this family, namely the WL-1 GNNs.

\paragraph{Finetune.} After the pretraining, the pretrained model is used to finetune on the downstream tasks. For molecule property prediction tasks, the graph-level representation obtained from the pretrained model is connected to linear classifiers to predict downstream task labels. The fine-tuning is performed in an end-to-end manner, where both the pretrained GNN and the linear classifiers are trainable. %: $y_G = f_F(h_G)$, where $h_G = \text{GNN}_{\theta}(X_G)$. the notation is terrible, so I'll just delete these for simplicity.

\paragraph{Graph pretraining objectives.} The primary goal of pretraining is to learn representations with robust transferable knowledge of graphs from the abundant pretraining data %through well-designed pretraining objectives. The learned knowledge can be 
and then generalize to downstream tasks with usually different supervision signals. Generally the pretraining objectives can be categorized into self-supervised and 
supervised ones. We present a brief overview of some representative objectives in the following sections. 

\subsection{Self-supervised (unsupervised) pretraining}
In self-supervised pretraining, the pretraining objective is designed to learn self-generated targets from the structure of the molecules, such as the type of nodes and edges, prediction of local context, graph partition, node clustering, occurrence of some functional groups, and etc. The predictive target can be node/edge level or entire graph level. We present some representative ones below:

{\color{red} %e both node and graph embeddings are of high-quality so that graph embeddings are robust and transferable across downstream tasks

%Therefore, while this type of pre-training is also very natural, it is beyond the scope of this paper and we leave its investigation for future work.

% When the GNN pre-training is finished, we fine-tune the pre-trained GNN model on downstream tasks. Specifically, we add linear classifiers on top of graph-level representations to predict downstream graph labels. The full model, i.e., the pre-trained GNN and downstream linear classifiers, is subsequently fine-tuned in an end-to-end manner. 

}
\subsubsection{Node Prediction}
Node prediction is a node-level classification task given the masked context of entire graph. Similar to \citet{devlin2018bert}, some portion of node attributes are masked and replaced with mask-specified indicators in the node input feature. After graph convolution, %aggregating neighbor representations, 
the embedding output from GNN is used to predict the true attribute of the node, e.g. atom type in molecular graphs, through a linear classifier on top of the node embedding. 
%The training objective is % $\min \sum_i \text{loss}(f_N(h_i), T_i)$ where $GNN$
%the   The node attribute is masked and the pretraining GNN is to predict the type of node (atom) 
%\cite{devlin2018bert}
%{\color{red} In Attribute Masking, we aim to capture domain knowledge by learning the regularities of the node/edge attributes distributed over graph structure.  Attribute Masking pre-training works as follows: We mask node/edge attributes and then we let GNNs predict those attributes (Devlin et al., 2019) based on neighboring structure.  Specifically, We randomly mask input node/edge attributes, for example atom types in molecular graphs, by replacing them with special masked indicators. We then apply GNNs to obtain the corresponding node/edge embeddings (edge embeddings can be obtained as a sum of node embeddings of the edge’s end nodes). Finally, a linear model is applied on top of embeddings to predict a masked node/edge attribute. }
%\begin{equation}
%   \min_{\theta, \gamma} \sum_i \text{Loss}(f_{N_\gamma}(h_i), T_i ) \quad \text{where } h_i = \text{GNN}_{\theta}(X_i)  
% \end{equation}


\subsubsection{Context Prediction}
Context prediction task is a sub-graph level task aiming at learning embedding that can represent the local subgraph surrounding a node. Generally it can be viewed as a masked task for substructure. Since it is essentially a structured prediction which can be difficult in general, \citet{hu2019strategies} leverages the adversarial learning to teach the model to distinguish the positive sub-graph embedding from the negative ones. 
%dot product of the two embedding. 
\citet{rong2020self} instead builds a dictionary of structures that captures the property of sub-graphs (e.g. type and quantity of neighbour nodes and bonds), and turns it into a multi-class classification problem. %using the embedding of node in the context center. %$h_i^K$. 
% {\color{red} In Context Prediction, we use subgraphs to predict their surrounding graph structures. Our goal
% is to pre-train a GNN so that it maps nodes appearing in similar structural contexts to nearby embeddings. 
% \textbf{GROVER} For the node/edge-level
% tasks, instead of predicting the node/edge type alone, GROVER randomly masks a local subgraph
% of the target node/edge and predicts this contextual property from node embeddings.
% The prediction target should reflect contextual information of the node/edge. Guided by these
% criteria, we present the tasks on both nodes and edges.
% They both try to predict the context-aware properties of
% the target node/edge within some local subgraph. 
% }
%\begin{equation}
%    % \quad
%    \min_{\theta} \sum_i \text{loss}(C_i, h_i) \quad \text{where } 
%    \quad
%    C_i = f_C(h_i, h_j: j\in \text{context}(i))
%\end{equation}
%where $f_c$ performs some transformation on context and target node to generate context embedding or labels. $f_C$ is embedding extraction function for \cite{hu2019strategies} and is label extraction for \cite{rong2020self}.

\subsubsection{Motif Prediction}
Motif prediction~\citep{rong2020self} is to %learn graph-level embedding through 
predict the existence of functional groups, such as benzene ring or hydroxyl. The motifs are extracted automatically from RDKit~\citep{landrum2016rdkit} . The motif prediction task is formulated as a graph-level multi-label binary classification task, where the graph embedding is used to jointly predict the occurrence of these semantic functional motifs.  %with one label for one motif. 
%Given a molecule, computational sorftware  can provide the supervised labels, and one label for one motif. Hence motif prediction task is a self-supervised task. The training objective is   
%
%\begin{equation}
%   \min_{\theta, \omega}  \text{Loss}(f_{M_\omega}(h_G), \{M_j: j = 1,2, .. m \} ) \quad \text{where } h_G = \text{GNN}_{\theta}(X) 
% \end{equation}
%where  $\{M_j: j = 1,2, .. m \}$ is a set of binary labels for $m$ motifs. $f_{M_\omega}$ is a multi-task linear classifier parameterized by $\omega$. 
 

%{\color{red} For the graph-level tasks, by incorporating the domain knowledge, GROVER extracts
%the semantic motifs existing in molecular graphs and predicts the occurrence of these motifs for a molecule from graph embeddings.

%fs are recurrent sub-graphs among the input graph data, which are prevalent in molecular graph data. One important class of motifs in molecules are functional groups, which encodes the rich domain knowledge of molecules and can be easily detected by the professional software, such as RDKit [27]. Formally, the motif prediction task can be formulated as a multi-label classificationproblem, where each motif corresponds to one label. }
\subsubsection{Contrastive learning}
Graph contrastive learning is to %, pretraining is performed through
maximize the agreement of two augmented views of the same graph, and minimize the agreement of different graphs. The optimization is conducted using contrastive loss in the latent embedding space \citep{you2020graph, hassani2020contrastive,zhu2021graph,wu2021self}. The augmentation function needs to transform graphs into realistic and novel augmentations without affecting semantic labels of the graphs. For example, the transformation can be small perturbations or modifications on node/edge embedding, drop of a few nodes or edges, and so on. These transformations enforce an underlying prior for contrastive learning, that is, local transformation does not change the semantic meaning of a graph.
%\begin{equation}
%\min_\theta -sim(h_G, h_G') + sum(h_G, h_G'') 
%\end{equation}
%\begin{equation}
%\text{where  } G'=f_A(G), G''=f_A(G_1), G1 \neq G
%\end{equation}
%where $sim$ is some similarity measure like cosine similarity. 

%The underlying prior enforced by it is that missing part of vertices does not affect the semantic meaning of



% {\color{red}

%  The main idea of contrastive learning is to make representations agree with
% each other under proper transformations, raising a recent surge of interest in visual representation
% learning

% In graph contrastive learning, pre-training is performed through maximizing the agreement
% between two augmented views of the graph via a contrastive loss in the latent space a

% contrastive learning aims to learn one or
% more encoders such that representations of similar graph
% instances agree with each other, and that representations
% of dissimilar graph instances disagree with each other. W

% }


% . A contrastive loss function L(·) is defined to enforce maximizing
% the consistency between positive pairs zi
% , zj compared with negative pairs. Here we utilize the
% normalized temperature-scaled cross entropy loss (NT-Xent) [51, 25, 52].
% During GNN pre-training, a minibatch of N graphs are randomly sampled and processed through
% contrastive learning, resulting in 2N augmented graphs and corresponding contrastive loss to optimize,
% where we re-annotate zi
%  zj as zn i  zn j for the nth graph in the minibatch. Negative pairs are not
% explicitly sampled but generated from the other N − 1 augmented graphs within the same minibatch
% as in [53, 18]. Denoting the cosine similarity function as sim(zn,i, zn,j ) = z
% T
% n,izn,j/kzn,ikkzn,jk,
% NT-Xent for the nth graph is defined as:
%  n = −log exp(sim(zn i, zn j )/tau )
% PN
% n0=1,n06=n
% exp(sim(zn,i, zn0
% ,j )/tau)
% , (3)
% where τ denotes the temperature parameter. The final loss is computed across all positive pairs in the
% minibatch. The proposed graph contrastive learning is summarized in Appendix A.}
%\vspace{-1mm}
\subsection{Supervised pretraining}
%{\color{red} We inject graph-level domain-specific knowledge into our pretrained embeddings by defining supervised graph-level prediction tasks In particular, we consider a practical method to pre-train graph representations: graph-level multi-task supervised pre-training to jointly predict a diverse set of supervised labels of individual graphs. }
Supervised pretraining aims to learn domain-specific graph-level knowledge from specifically designed pretraining tasks. For molecular application, the supervised labels are generated from a diverse set of functional studies like biochemical assays. The pretrainning task is to perform multiple binary classification and jointly learn the supervised labels. Although the pretraining mainly refers to unsupervised or self-supervised methods as they are not limited by the requirement of supervised labels, supervised pretraining is still a great source to investigate the graph pretraining in general.


\begin{table*}[t]
\small
\centering
%\vspace{-2mm}
\caption{\textbf{Self-supervised} + Rich feature + Balanced Scaffold Split.  No pretrain has an average value of 78.0\% over all 5 datasets. \label{tab:unsupervised-obj}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
\Xhline{2\arrayrulewidth}
%\hline
Methods           & \textbf{BBBP}            & \textbf{BACE}                  & \textbf{TOX21}           & \textbf{TOXCAST}        & \textbf{SIDER  }  &    \textbf{AVE GAIN}    \\ %\midrule %\hline
\Xhline{2\arrayrulewidth}
\nopretrain      & 92.23($\pm$3.07) & 87.43($\pm$1.63)     & 79.20($\pm$1.99)  & 69.13($\pm$0.55) & 61.92($\pm$0.89) & 0($\pm$1.626)\\
\masktask        & 92.24($\pm$2.76) & 87.32($\pm$1.67)     & 79.57($\pm$2.03) & 69.77($\pm$0.13) & 61.62($\pm$1.12) & 0.122($\pm$1.542)\\
\contexttask     & 92.68($\pm$1.19) & 86.98($\pm$1.26)     & 79.05($\pm$2.51) & 70.18($\pm$0.44) & 61.65($\pm$0.77) & 0.126($\pm$1.234)\\
\motiftask       & 92.63($\pm$1.19) & 87.16($\pm$1.66)     & 79.22($\pm$2.38) & 69.09($\pm$0.07) & 62.45($\pm$1.25) & 0.128($\pm$1.310)\\  
\contrastivetask  & 92.31($\pm$1.58)& 86.67($\pm$2.40)     & 78.45($\pm$2.44) & 68.37($\pm$0.80) & 61.22($\pm$1.20) & -0.578($\pm$1.684) \\ 
%\hline
\Xhline{2\arrayrulewidth}
%\vspace{-6mm}
\end{tabular}%
}
\vspace{-2mm}
\end{table*}

\begin{table*}[h]
\small
%\caption{Supervised Pretraining Objectives on Downstream Task Accuracy (\%)}
%\vspace{-2mm}
\centering
\caption{\textbf{Supervised} + Rich feature + Balanced Scaffold.  No pretrain has an average AUC of 78.0\%. \label{tab:super-obj}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
%\hline
\Xhline{2\arrayrulewidth}
Methods                    & \textbf{BBBP}   & \textbf{BACE}   & \textbf{TOX21}   & \textbf{TOXCAST} & \textbf{SIDER}  &    \textbf{AVE GAIN}   \\ 
\Xhline{2\arrayrulewidth}
\nopretrain      & 92.23($\pm$3.07) & 87.43($\pm$1.63) & 79.2($\pm$1.99)  & 69.13($\pm$0.55) & 61.92($\pm$0.89) & 0($\pm$1.626)\\
\supervisedtask  & 91.65($\pm$2.11) & 86.91($\pm$1.86) & 81.13($\pm$2.39) & 71.64($\pm$0.46) & 62.14($\pm$1.13) & 0.712($\pm$1.590)\\
\supervisedmasktask     & \textbf{93.43($\pm$2.50)} & 86.90($\pm$2.04) & \textbf{81.93($\pm$1.79)} & 71.66($\pm$0.73) & 62.68($\pm$1.82) & 1.338($\pm$1.776)\\
\supervisedcontexttask& 92.27($\pm$1.57) & \textbf{88.72($\pm$1.68)} & 81.71($\pm$1.79)   & \textbf{72.19($\pm$0.79)}  & \textbf{63.21($\pm$1.49)}  & 1.638($\pm$1.464) \\ 
\Xhline{2\arrayrulewidth}
%\vspace{-10mm}
\end{tabular}%
}
\vspace{-2mm}
\end{table*}

\begin{table*}[t]
\small
%\vspace{-3mm}
\centering
\caption{Self-supervised + Rich feature + \textbf{Scaffold}. No pretrain has an average ROC-AUC of 71.8\% over all benckmark datasets. \label{tab:split}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
%\hline
\Xhline{2\arrayrulewidth}
Methods        & \textbf{BBBP}             & \textbf{BACE}    & \textbf{TOX21}    & \textbf{TOXCAST} & \textbf{SIDER} &    \textbf{AVE GAIN}   \\ %\hline
\Xhline{2\arrayrulewidth}
%\nopretrain      & \textbf{75.13($\pm$1.08)} & 79.79($\pm$1.18) &  76.06($\pm$0.20) & 66.1($\pm$0.42)  & 61.21($\pm$0.76) \\
\nopretrain      & 74.83($\pm$0.73) & 80.10($\pm$0.42) & 75.86($\pm$0.58)  & 65.95($\pm$0.15) & 62.30($\pm$1.14) & 0($\pm$0.579)\\
\masktask        & 73.45($\pm$0.27) & 83.66($\pm$0.75) & 75.30($\pm$0.37)  & 66.50($\pm$0.06) & 65.08($\pm$0.12) & 0.990($\pm$0.323)\\
\contexttask     & 74.10($\pm$0.22) & 81.87($\pm$0.49) &75.37($\pm$0.11)   & 66.86($\pm$0.07) & 62.84($\pm$0.46) & 0.400($\pm$0.280)\\
\motiftask       & 73.65($\pm$0.36) & 80.58($\pm$2.04) & 74.55($\pm$0.79)  & 65.63($\pm$0.07) & 64.05($\pm$0.23) & -0.116($\pm$0.766)\\
\contrastivetask & 73.32($\pm$2.38) & 80.51($\pm$0.80) & 74.55($\pm$0.22)  & 65.70($\pm$0.09) & 64.39($\pm$0.63) & -0.114($\pm$0.513)\\ 
%\hline
\Xhline{2\arrayrulewidth}
%\vspace{-6mm}
\end{tabular}%

}
%\caption{Scaffold split + rich feature}
\end{table*}

\begin{table*}[t]
\small
\centering
%\vspace{-3mm}
\caption{Supervised %+ Self-supervised 
+ Rich feature + \textbf{Scaffold}. No pretrain get 71.8\% average ROC-AUC. \label{tab:feature-scaffold-richfeature-supervised}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccr}
%\hline
\Xhline{2\arrayrulewidth}
Methods & \textbf{BBBP}              & \textbf{BACE}     & \textbf{TOX21}    & \textbf{TOXCAST}      & \textbf{SIDER} &    \textbf{AVE GAIN}  \\ %\hline
\Xhline{2\arrayrulewidth}
\nopretrain                 & \textbf{74.83($\pm$0.73)}     & 80.10($\pm$0.42)          & 75.86($\pm$0.58)          & 65.95($\pm$0.15)          & 62.30($\pm$1.14)           & 0($\pm$0.604) \\
\supervisedtask             & 72.79( $\pm$ 0.7)             & 83.23($\pm$0.67)          & 77.66($\pm$0.08)          & 67.72($\pm$0.13)          & 65.34($\pm$0.17)           & 1.540($\pm$0.350) \\
\supervisedmasktask         & 73.38($\pm$0.55)              & \textbf{84.42($\pm$0.27)} & \textbf{77.85($\pm$0.24)} & \textbf{67.14($\pm$0.28)} & 64.06($\pm$0.28)           & 1.562($\pm$0.324) \\
\supervisedcontexttask      & 73.81($\pm$0.52)              & \ 84.35($\pm$0.93)        & 77.11($\pm$0.14)          & 67.87($\pm$0.08)          & \textbf{65.19($\pm$0.17)}  & 1.858($\pm$0.368)  \\ 
%\hline
\Xhline{2\arrayrulewidth}
%\vspace{-7mm}
\end{tabular}%
}
\end{table*}

==> [NeurIPS2022] Graph pretraining/introduction.tex <==
\section{Introduction}





%The gain obtained by pretraining, mainly refer to supervised pretraining,  is larger in lower accuracy region (i.e. on scaffold split, basic feature) than that on high accuracy region (i.e. on balanced scaffold, rich feature). By using rich features, the gain achieved by supervised pretraining is reduced. 


%We reach a conclusion that unsupervised pretraining strategies do not have significance improvements over no pretraining, whereas supervised pretrainig improves more on low accuracy region, whereas the effect is reduced in higher accuracy region (i.e.achieved by balanced split or rich feature). 

Graph neural networks (GNNs)
, due to their effectiveness,
have been adopted to model a wide range of structured data, such as social networks, road graphs, citation networks, etc. Molecule modeling is one of these important applications, where it serves as the foundation of biomedicine and nurturing techniques like novel drug discovery. However, labeling biomedical data are usually time-consuming and expensive and thus task-specific labels are extremely inadequate. This poses a big challenge to the field. Recently, inspired by the remarkable success of self-supervised pretraining from natural language processing~\citep{devlin2018bert, brown2020language,wei2021finetuned} and computer vision domains~\citep{he2020moco,chen2020simple}, researchers start trying to apply the pretrain-finetune paradigm to molecule modeling with GNN, hoping to boost the performance of various molecular tasks by pretraining the model on the enormous unlabeled data.
% Therefore, self-supervised pretraining is indeed very attractive as it might potentially alleviate this issue.
% In this paper, we are particularly interested in the GNN pretraining for molecule presentations. 
% The past few years have witnessed the remarkable achievements of self-supervised pretraining in many scientific fields, such as computer vision \adamsyuwei{should cite Kaiming He "Moco" and Ting Chen "SimCLR"} \citep{dosovitskiy2020image,dai2021coatnet,chen2020simple} and natural language processing \adamsyuwei{should cite Jacob Devlin "BERT"} \citep{raffel2019exploring, wei2021finetuned,brown2020language}. Recently, researchers start trying to apply the pretrain-finetune paradigm to other less explored domains with abundant unlabeled data, hoping to replicate the success of self-supervised pretraining.
% exploiting opportunities to accelerate the process of transferring robust generalizable knowledge obtained from abundant pretraining data to benefit realistic tasks in drug discovery and biomedical domain (molecules).
% Molecules are usually abstracted as graphs to preserve its rich structure information. Self-supervised graph pretraining is of particular interest because: First, task-specific labels are inadequate, as biomedical labeling requires time and resource-intensive wet-lab experiments, and pretraining can be a good option to alleviate the issue as it is in computer vision \citep{chen2020simple,sohn2020fixmatch}; Second, models suffer from poor generalization capability in chemical space. Pretraining can initialize graph neural networks models to a ``better'' basin around a good local optima that can better generalize. % Encouraging results [cite??] have been reported recently on the efficacy of GNN pretraining in molecule representation, claiming downstream applications indeed benefit from finetuning the pretrained networks.
For instance, %a large variety of 
many methods have been proposed~\citep{xie2021self,wu2021self}, where significant performance improvements are claimed
% due to well designed pretraining objectives and 
by pretraining on large scale datasets \citep{hu2019strategies, rong2020self,  you2020graph, you2020does, zhu2021graph}. Despite of the promising results, %we find research on investigating the factors for the improvement are still at a nascent stage. Based on our experiments, 
we find that reproducing some of these outstanding gains via graph pretraining can be non-trivial, and sometimes the improvement largely relies on the experimental setup and the extensive hyper-parameter tuning of downstream tasks, rather than the design of pretraining objectives. These observations motivate us to rethink the effectiveness of graph pretraining with unsupervised or self-supervised objectives, and investigate what factors would influence the effectiveness of self-supervised graph pretraining.
% and to investigate what possibly influences the effectiveness. % All of these motivate this paper.

\begin{figure*}[ht]
\includegraphics[width=1.0\textwidth]{figs/graph_pretrain_pipeline.drawio_morestraws}
\caption{A typical pipeline for graph pretraining and deployment for downstream applications. \label{fig:pipeline}}
\end{figure*}


In this paper, we perform systematic studies to
assess the performance of popular graph pretraining objectives on different types of datasets, and exploit various confounding components in experimental setup in deciding the performance of downstream tasks with or without pretraining. 
Here, we restrict our studies to small molecular graphs, as opposed to other application domains, such as social networks or citation graphs. The key insights and take-aways of this paper are:
\begin{itemize}[leftmargin=*]%[noitemsep,topsep=1pt,parsep=1pt,partopsep=0pt, leftmargin=*]
    \item Among the pretraining tasks we evaluated, the self-supervised pretraining alone does not provide statistically significant improvements over non-pretrained methods on downstream tasks.
    \item When additional supervised pretraining step is conducted after self-supervised pretraining, we observe statistically significant improvements. However, the gain becomes marginal on some specific data splits or diminishes if richer features are introduced.
    \item Beyond data splits and hand-crafted features, the usefulness of graph pretraining is also sensitive to the experimental hyperparameters, such as learning rates and number of study repeats. Different setups can lead to opposite conclusions. 
    \item In conclusion, different from the previous works, we do not observe clear and unconditional gains achieved by graph pretraining on molecular representation, indicating it is still too early to conclude graph pretraining is effective in molecular domain.
    \item  We investigate the reason of above and hypothesize that the complexity of some pretraining methods on molecules is insufficient, leading to less transferable knowledge for downstream tasks.
\end{itemize}

Despite the overall negative results we obtained, the main goal of this paper is not to discourage the pretraining research for small molecules. Instead, we hope to raise the attention on different aspects of experiments and the role of simple hand-crafted features, so as to provide useful information for designing better pretraining approaches. Below we first introduce the background of GNN and its pretraining in \secref{sec:gnn_pretrain}, and then our experimental design and results in \secref{sec:exp_framework} and \secref{sec:results}, respectively. Finally we conclude with our findings and the limitations in \secref{sec:summary} and  \secref{sec:limitation}.
% \begin{itemize}[noitemsep,topsep=1pt,parsep=1pt,partopsep=0pt, leftmargin=*]
%     \item Model: we choose GIN
%     \item Pretraining datatset: Zinc
%     \item scaffold: we use balanced scaffold, as ...
% \end{itemize}

% Systematic study is performed to
% assess the performance of contrasting different augmentations on various types of datasets, revealing
% the rationale of the performances and providing the guidance to adopt the framework for specific
% datasets. 



% However, the effectiveness of these methods remains unclear. The authors found to reproduce some of the reported large gain of graph pretraining results are non-trivial, if not unlikely. The good performance of downstream is largely relied on extensive hyper parameters tuning, which 

% %The main goal of this study was therefore to compare the performance of proposed graph pretraining methods and 


% %Grover \citep{rong2020self}

% %ICLR \citep{hu2019strategies}


% The insights
% we gained are that well-designed self-supervision losses and largely-expressive
% pre-trained models enjoy the significant potential on performance boosting.


% Existing work claims: The success of the pre-training model crucially depends on the design of self-supervision tasks.

% Molecules can be naturally represented as graph to preserve rich structure information,  graph-pretraining on molecule domain has raised surge of interest and many promising 

% The robust transferable knowledge learned from the abundant pretraining data generalize to other downstream tasks of interest 
% {\color{red}
% [\textbf{good sentences copied from other paper, rephrase!}] \\


% Inspired by the remarkable achievements of deep learning in many scientific domains, such as computer vision, natural language processing, and social networks, researchers
% are exploiting deep learning approaches to accelerate the process of drug discovery and reduce costs
% by facilitating the rapid identification of molecules. Molecules can be naturally represented by
% molecular graphs which preserve rich structural information. Therefore, supervised deep learning of
% graphs, especially with Graph Neural Networks(GNNs) have shown promising results in
% many tasks, such as molecular property prediction and virtual screening.


% Despite the fruitful progress, two issues still impede the usage of deep learning in real scenarios:
% (1) insufficient labeled data for molecular tasks; (2) poor generalization capability of models in the
% enormous chemical space. Different from other domains (such as image classification) that have
% rich-source labeled data, getting labels of molecular property requires wet-lab experiments which is
% time-consuming and resource-costly. As a consequence, most public molecular benchmarks contain
% far-from-adequate labels. Conducting deep learning on these benchmarks is prone to over-fitting and
% the learned model can hardly cope with the out-of-distribution molecules.

% Recently, GNNs have received a surge of interest in various
% domains, such as knowledge graph, social networks and drug discovery.

% Generalizable, transferrable, and robust representation learning on graph-structured
% data remains a challenge for current graph neural networks (GNNs). Unlike what
% has been developed for convolutional neural networks (CNNs) for image data,
% self-supervised learning and pre-training are less explored for GNNs. In this
% paper, we propose a graph contrastive learning (GraphCL) framework for learning
% unsupervised representations of graph data. W

% The results show that, even without tuning augmentation
% extents nor using sophisticated GNN architectures, our GraphCL framework can
% produce graph representations of similar or better generalizability, transferrability,
% and robustness compared to state-of-the-art methods. 

% We however argue for the necessity of exploring GNN pre-training schemes. Task-specific labels
% can be extremely scarce for graph datasets (e.g. in biology and chemistry labeling through wet-lab
% experiments is often resource- and time-intensive) [15, 9], and pre-training can be a promising
% technique to mitigate the issue, as it does in convolutional neural networks (CNNs) [16, 17, 18]. As to
% the conjectured reasons for the lack of GNN pre-training: first, real-world graph data can be huge and
% even benchmark datasets are recently getting larger [12, 19]; second, even for shallow models, pretraining could initialize parameters in a “better" attraction basin around a local minimum associated
% with better generalization [11]. Therefore, we emphasize the significance of GNN pre-training.

% In comparison, contrastive
% learning aims to learn representations by maximizing feature consistency under differently augmented
% views, that exploit data- or task-specific augmentations [33], to inject the desired feature invariance.

% as graphs are abstracted representations of raw data with
% diverse nature (e.g. molecules made of chemically-bonded atoms and networks of socially-interacting
% people). It is thus difficult to design a GNN pre-training scheme generically beneficial to down-stream
% tasks.

% overcome the aforementioned
% limitations of proximity-based pre-training methods

% h imposes certain prior
% over graph data and parameterized for the extent and pattern. (ii) Utilizing them to obtain correlated
% views, we propose a novel graph contrastive learning framework (GraphCL) for GNN pre-training, 

% Systematic study is performed to
% assess the performance of contrasting different augmentations on various types of datasets, revealing
% the rationale of the performances and providing the guidance to adopt the framework for specific
% datasets. 

% Utilizing them to obtain correlated
% views, we propose a novel graph contrastive learning framework (GraphCL) for GNN pre-training, so
% that representations invariant to specialized perturbations can be learned for diverse graph-structured
% data.



% The main idea of contrastive learning is to make representations agree with
% each other under proper transformations, raising a recent surge of interest in visual representation
% learning [45, 25, 26, 27, 18]. On a parallel note, for graph data, traditional methods trying to
% reconstruct the adjacency information of vertic

% %Data augmentation aims at creating novel and realistically rational data through applying certain transformation without affecting the semantics label. I

% graph datasets are abstracted from diverse fields and therefore there may not be universally
% appropriate data augmentation as those for images.

% node dropping will randomly discard certain portion of vertices

% s the challenge of data heterogeneity in graphs.

% contrastive learning has renewed a surge of interest

% Motivated by recent contrastive learning developments in visual representation learning 

% %In graph contrastive learning, pre-training is performed through maximizing the agreement
% %between two augmented views of the same graph via a contrastive loss in the latent space a

% Therefore, a well designed pre-training
% framework is needed to capture highly heterogeneous information in graph-structured data.

%  It implies that the semantic meaning of G
 


% several works aim to establish a pre-trained model directly on the graph
% representations of molecules.


% An effective approach to this
% challenge is to pre-train a model on related tasks where data is abundant, and then
% fine-tune it on a downstream task of interest. 

% While pre-training has been effective
% in many language and vision domains, it remains an open question how to effectively use pre-training on graph datasets. 

% graph
% data from real-world applications often contain out-of-distribution samples, meaning that graphs in
% the training set are structurally very different from graphs in the test set. Out-of-distribution prediction
% is common in real-world graph datasets


%  The key idea is to use easily accessible
% node-level information and encourage GNNs to capture domain-specific knowledge about nodes and
% edges, in addition to graph-level knowledge. This helps the GNN to learn useful representations
% at both global and local levels




% Recently self-supervised learning (SSL) techniques have gained success in many domains, e.g., visual, natural language processing, and robotics, where SSL methods even outperform their supervised counterparts. However, the development of SSL in the graph domain is still at a nascent stage.

% achieved remarkable success

% Based on how the pretext training tasks are designed,
% SSL methods can be divided into two categories; namely
% contrastive models and predictive models. The major difference between the two categories is that contrastive models
% require data-data pairs for training, while predictive models
% require data-label pairs, where the labels are self-generated
% from the data




% To alleviate this issue, the key insight 

% the combined strategy produces much more transferable graph representations and robustly improves
% downstream performance 


% How to obtain informative representations of molecules is a crucial prerequisite
% in AI-driven drug design and discovery. Recent researches abstract molecules as
% graphs and employ Graph Neural Networks (GNNs) for molecular representation
% learning. Nevertheless, two issues impede the usage of GNNs in real scenarios:
% (1) insufficient labeled molecules for supervised training; (2) poor generalization
% capability to new-synthesized molecules. To address them both, w

% can learn rich structural and semantic information of molecules from enormous unlabelled molecular data.

% The insights
% we gained are that well-designed self-supervision losses and largely-expressive
% pre-trained models enjoy the significant potential on performance boosting.


% Existing work claims: The success of the pre-training model crucially depends on the design of self-supervision tasks.

% abundant labeled data,

% d, as advocated in  



% The
% primary goal of SSL is to learn transferable knowledge from
% abundant unlabeled data with well-designed pretext tasks
% and then generalize the learned knowledge to downstream
% tasks with specific supervision signals.

% Inevitably,
% such divergence will significantly hurt the generalization of
% learned models. Therefore, it is crucial to reconsider the objectives of pretext tasks to better match that of downstream
% tasks and make them consistent with each other.

%  The main idea of contrastive learning is to make representations agree with
% each other under proper transformations, raising a recent surge of interest in visual representation
% learning

% }



% \begin{itemize}
%     \item Pretraining \& success
%     \item Graph pretraining \& existing work for molecuelar domain 
%     \item Overview \& contribution of this work
% \end{itemize}

% Pretraining has achieved success on a variety of applications, text (NLP), image, etc. Pretraining is to learn representation 
% The advantage of pretraining is one can learn useful representation by leveraging on a large amount of pretraining data. In order to a useful prepresentation that can benefit downstream tasks, different pretraining tasks 




%Graph pretraining is to perform pretraining to utilize graph structure, such as vertex and edges. For example, masking pretraining. masking node and predict the node label, masking edge to predict edge label. Context prediction: 



%However, we investigate several pretraining tasks and the performance compared with downstream task without pretraining to evaluate different performance of downstream tasks.  tested a few


%pretraining and downstream supervision has different objectives. 

% 0 Introduction 
% 1 experiment details 
%     comments / conclusion 
% 2 summery of conclusion/ take away 
% 3 analysis hypothesis 
% 4 limitations 

%The design of pretraining task is 

%A large variety of pretraining methods for molecular application have been proposed, including unsupervised pretraining, supervised pretraining, contrastive learning. However, the effectiveness of these methods remains unclear. The authors found to reproduce some of the reported large gain of graph pretraining results are non-trivial, if not unlikely. The good performance of downstream is largely relied on extensive hyper parameters tuning, which alarms us to rethink how effectiveness self-supervised graph pretraining is and what influence the effectiveness of graph pretraining. All these motivate this paper. 

%The main goal of this study was therefore to compare the performance of proposed graph pretraining methods and 


%Grover \citep{rong2020self}

%ICLR \citep{hu2019strategies}

 
%ICLR requires electronic submissions, processed by
%\url{https://openreview.net/}. See ICLR's website for more instructions.

%If your paper is ultimately accepted, the statement {\tt
%  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
%format to the camera ready requirements.

%The format for the submissions is a variant of the NeurIPS format.
%Please read carefully the instructions below, and follow them
%faithfully.

%\section{Overview: Investigate performance of pretraining on downstream tasks}
%We investigate the following aspects that may influence the performance of pretraining on downstream tasks. We summarize in the following overview. 

% \begin{itemize}
%     \item[$\circ$] Pretraining objectives 
%     \begin{itemize}
%         \item Masking 
%             \begin{itemize}
%                 \item[-] Node
%                 \item Context 
%              \end{itemize}
%         \item[$\circ$]  Contrastive 
%             \begin{itemize}
%                 \item Augmentations 
%                 \item Reaction
%             \end{itemize}
%         \item[$\circ$] Graph-level supervision
%     \end{itemize}
%     \item Split
%     \item Feature
%     \item Architecture
%     \item Data scale
    
    
% \end{itemize}

 


% \begin{enumerate}
%     \item Pretraining objectives 
%         \begin{enumerate}
%             \item Masking 
%                 \begin{enumerate}
%                     \item Node
%                     \item Context 
%                 \end{enumerate}
%             \item  Contrastive 
%                 \begin{enumerate}
%                     \item Augmentations 
%                     \item Reaction
%                 \end{enumerate}
%             \item Graph-level supervision
%                 \begin{enumerate}
%                     \item Supervosed learning
%                 \end{enumerate}
        
%         \end{enumerate}
%     \item Split
%         \begin{enumerate}
%             %\item Uniform
%             \item Balanced scaffold 
%             \item Scaffold 
%         \end{enumerate}
    
%     \item Feature
%         \begin{enumerate}
%             \item Basic feature
%             \item Rich feature 
%         \end{enumerate}
%     \item Architecture
%         \begin{enumerate}
%             \item GIN
%             \item Graph transformer
%             \item graphsage
%         \end{enumerate}
%     \item Data scale
    
%         \begin{enumerate}
%             \item 2M 
%             \item SAVI (1,063,045,046)
%         \end{enumerate}
    
    
% \end{enumerate}




==> [NeurIPS2022] Graph pretraining/limitation.tex <==
%\vspace{-3mm}
\section{Limitations of current study}
\label{sec:limitation}
%\vspace{-3mm}
Although we have tried our best to design a comprehensive study on the effectiveness of graph pretraining for molecular representation, there are still limitations we want to point out. Due to the limited time and resources we have, we are not able to fully cover the whole picture of the current pretraining paradigm in graph neural networks. Nevertheless, we list them here in hope of preventing the over-generalization of our conclusion.
\begin{itemize}[leftmargin=*,nosep]
    \item \textit{Distribution of graphs}. Our study focuses on pretraining for small molecule graph inductive representation learning. Recently there are works on pretraining transductive representation learning~\citep{you2020does} on large graphs~\citep{hu2020gpt}, where our conclusion may not be directly extended to these cases. 
    \item \textit{Graph architectures}. GNN is a popular research field where many new architectures with probable expressiveness are/will be proposed. The results we have shown are on two representative 1-WL GNNs. It can be possible that the latest advances of deep GNN~\citep{liu2020towards} and Transformer-based GNN~\citep{ying2021transformers, chen2022structure, kim2022pure} might yield different results.
    \item \textit{Learning objectives}. Although we have presented results with different types of self-supervised losses, there are still many variants of each type that we did not explore, like different variants~\citep{sun2021mocl, xia2022simgrace} of contrastive learning. Also, multi-task learning of different self-supervised objectives might be another direction for further exploration.
    \item \textit{Downstream datasets}. We obtained our conclusion mainly on the datasets from MoleculeNet~\citep{wu2018moleculenet}. Datasets like Alchemy~\citep{chen2019alchemy} and drug-target Interaction~\citep{liu2021pre} may show different results.
\end{itemize}


==> [NeurIPS2022] Graph pretraining/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
% \newcommand{\figleft}{{\em (Left)}}
% \newcommand{\figcenter}{{\em (Center)}}
% \newcommand{\figright}{{\em (Right)}}
% \newcommand{\figtop}{{\em (Top)}}
% \newcommand{\figbottom}{{\em (Bottom)}}
% \newcommand{\captiona}{{\em (a)}}
% \newcommand{\captionb}{{\em (b)}}
% \newcommand{\captionc}{{\em (c)}}
% \newcommand{\captiond}{{\em (d)}}


% Highlight a newly defined term
%\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
%\def\secref#1{section~\ref{#1}}
\def\secref#1{Section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
% \newcommand{\train}{\mathcal{D}}
% \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
%\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
%\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
 
 % The true underlying data generating distribution
% \newcommand{\pdata}{p_{\rm{data}}}
% % The empirical distribution defined by the training set
% \newcommand{\ptrain}{\hat{p}_{\rm{data}}}
% \newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% % The model distribution
% \newcommand{\pmodel}{p_{\rm{model}}}
% \newcommand{\Pmodel}{P_{\rm{model}}}
% \newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% % Stochastic autoencoder distributions
% \newcommand{\pencode}{p_{\rm{encoder}}}
% \newcommand{\pdecode}{p_{\rm{decoder}}}
% \newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
% \newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\emp}{\tilde{p}}
% \newcommand{\lr}{\alpha}
% \newcommand{\reg}{\lambda}
% \newcommand{\rect}{\mathrm{rectifier}}
% \newcommand{\softmax}{\mathrm{softmax}}
% \newcommand{\sigmoid}{\sigma}
% \newcommand{\softplus}{\zeta}
% \newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
% \newcommand{\standarderror}{\mathrm{SE}}
% \newcommand{\Cov}{\mathrm{Cov}}
% % Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% % But then they seem to use $L^2$ for vectors throughout the site, and so does
% % wikipedia.
% \newcommand{\normlzero}{L^0}
% \newcommand{\normlone}{L^1}
% \newcommand{\normltwo}{L^2}
% \newcommand{\normlp}{L^p}
% \newcommand{\normmax}{L^\infty}

% \newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
% \let\ab\allowbreak

% % customer 
% \newcommand{\rbr}[1]{\left(#1\right)}
% %\newcommand{\chapref}[1]{Chapter~\ref{#1}}
%\newcommand{\secref}[1]{Section~\ref{#1}}
% %\newcommand{\secref}[1]{Sec~\ref{#1}}
% \newcommand{\eqnref}[1]{Eq~(\ref{#1})}
% \newcommand{\eqnsref}[1]{Eqns~(\ref{#1})}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
% %\newcommand{\algref}[1]{Algorithm~\ref{#1}}
% \newcommand{\lemref}[1]{Lemma~\ref{#1}}
% \newcommand{\propref}[1]{Proposition~\ref{#1}}
% \newcommand{\thmref}[1]{Theorem~\ref{#1}}
% \newcommand{\asmpref}[1]{Assumption~\ref{#1}}
%\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
% \newcommand{\corref}[1]{Corollary~\ref{#1}}
% %\renewcommand{\algorithmiccomment}[1]{\bgroup\hfill//~#1\egroup}

% \newcommand{\ea}{\emph{et al.}}
% \newcommand{\eg}{\emph{e.g.}}
% \newcommand{\ie}{\emph{i.e.}}
% \newcommand{\iid}{\emph{i.i.d.}}
% \newcommand{\etc}{\emph{etc.}}

% %\newcommand{\rbr}[1]{\left(#1\right)}
% \newcommand{\sbr}[1]{\left[#1\right]}
% \newcommand{\cbr}[1]{\left\{#1\right\}}

% \newcommand{\EE}{\mathbb{E}} % Expectation

% \newcommand{\II}{\mathbb{I}} % Indicator
% \newcommand{\Pscr}{\mathscr{P}}
% \newcommand{\RR}{\mathbb{R}} % Real numbers
% \newcommand{\Xcal}{\mathcal{X}}
% %\newcommand{\Tcalb}{\bm{\Tcal}}
% \newcommand{\Tcal}{{\mathcal{T}}}



==> [NeurIPS2022] Graph pretraining/results.tex <==
%\vspace{-3mm}
\section{Results}
\label{sec:results}
%\vspace{-3mm}
In this section, we present the results and discussions for a set of experiments designed with the protocols in \Secref{sec:protocol}. \tabref{tab:summary-table} summarizes the experimental configurations for each following table. We will elaborate on them in the following sections. 
Due to space limit, we defer our investigation on different GNN architectures to appendix (\secref{sec：gnn}).

%\input{summary_table}
%\vspace{-2mm}
\subsection{Vanilla configuration}
%\vspace{-1mm}
We choose the \emph{vanilla configuration} with the settings from existing works~\citep{hu2019strategies, rong2020self}. Specifically, we use the \textbf{rich feature} with \textbf{GIN} backbone, pretrained on \textbf{ZINC15} when pretraining is applied, and evaluate on the \textbf{Balanced Scaffold Split} for downstream tasks. One important baseline is without pretraining. For the ease of comparison, we include the results without pretraining in each table.
%\vspace{-2mm}
\subsection{Self-supervised pretraining objectives}
We compare the results pretrained with different self-supervised pretraining objectives. As is presented in \Secref{sec:design_choice}, we consider four representative types of pretraining objectives. For the ease of comparing the performance, we only consider one objective at a time, instead of mixing different pretraining objectives to obtain a multi-task pretrained model. 
\tabref{tab:unsupervised-obj} shows the performance on downstream molecule property prediction benchmarks with models initialized from different pretraining objectives. The relative average gain compared to the one without pretraining is not statistically significant, i.e., not larger than the standard deviations of multiple runs. All the four different objectives obtain similar gains/loses regardless of very different designs. To fully understand the effect of self-supervised pretraining on molecule representation, we further investigate the performance of different pretraining objectives in combination with other factors, such as input features or data splits, as described in the following sections. 
%\vspace{-2mm}
\subsection{Supervised pretraining objectives}
In addition to the self-supervised objectives, we study the potential benefits with supervised pretraining. Unlike the self-supervised setting where the molecule graphs themselves are used for pretraining, the supervised pretraining requires extra cost of data labeling, and thus is not scalable for large scale pretraining. In this paper, we present the results with supervised pretraining alone, as well as the joint pretraining. e.g. pretrain with self-supervised objective and followed by supervised pretraining, in \tabref{tab:super-obj}. We can see with the supervised pretraining, one can improve the downstream performance, which aligns with the observation from \citet{hu2019strategies}. Our hypothesis is that, supervised pretraining is helpful when the pretraining tasks are closely aligned with the downstream tasks. In particular, the bio-activity labels provided by ChEMBL is highly related to the drug discovery purpose and drug discovery properties are the major topics evaluated in the downstream tasks. %\tabref{tab:super-obj} shows that the downstream tasks that are directly measuring biophysical property for drug discovery, such as toxicity, obtain the largest performance improvement from ChEMBL pretraining (e.g. TOXCAST and TOX21). %On the contrary, tasks that do not directly measure drug-able property such as BBBP (predict blood-brain barrier) achieve less gain.  
Therefore, the positive correlation between the pretraining supervision and downstream tasks contribute the most to the performance improvement of downstream tasks. %Based on this fact, the requirement for additional labels and the close alignment between pretraining and downstream tasks can limite the useage of supervised pretraining. 
%\vspace{-3mm}
\subsection{Data split on downstream tasks}
Molecular data is usually diverse and limited, so chemists are particularly interested in the generalization ability of GNNs on out of distribution data. Also due to the same reason (i.e. limited and diverse data), the variance in performance of different splits is significant, which poses challenges on robust evaluation. In \emph{vanilla configuration} we use the balanced scaffold split, and here we show additional results with the \textbf{scaffold} split, which is a deterministic data split that makes the train/valid/test set differ from each other the most.  \tabref{tab:split} and \tabref{tab:feature-scaffold-richfeature-supervised} respectively present the results using scaffold split with self-supervised without and with additional supervised pretraining. Compared with \tabref{tab:unsupervised-obj} and \tabref{tab:super-obj}, it is clear to see that \tabref{tab:split} and \tabref{tab:feature-scaffold-richfeature-supervised} have significantly lower ROC-AUC. Specifically the AUC drops 6.2\% on average for all benchmarks without pretraining. On the other hand, we can see if we compare \tabref{tab:split} with \tabref{tab:unsupervised-obj}, or \tabref{tab:feature-scaffold-richfeature-supervised} with \tabref{tab:super-obj} respectively, the gain of pretraining is more significant on the \textbf{scaffold} split. We 
speculate the reason for the improvement of scaffold split is that the initialization of neural network parameters (e.g. from pretraining) are typically critical for the out-of-distribution generalization (e.g. scaffold split). Similar observations have also been studied in the meta-learning literature~\citep{finn2017model}.  Although the gain with supervised pretraining is significant in \tabref{tab:feature-scaffold-richfeature-supervised},  the effect of self-supervised pretraining is mixed in \tabref{tab:split}. This indicates the effectiveness of self-supervised pretraining on scaffold split is not significant enough to claim ``very helpful''.  
%\vspace{-3mm}
\subsection{Graph features}
%\vspace{-2mm}
So far we have presented the results with rich features. Now we want to see how those basic features used in~\citet{hu2019strategies} affect the outcome. \tabref{tab:Balanced scaffold + basic feature + unsupervised} and \tabref{tab:Balanced scaffold + basic feature + supervised} show the test ROC-AUC (\%) performance with {\it basic features} on the balanced scaffold splits using self-supervised or supervised pretraining objectives, respectively. \tabref{tab:Scaffold + basic feature + unsupervised} and \tabref{tab:Scaffold + basic feature +  supervised} show the same results but on scaffold split. %instead. 

In a nutshell, without pretraining, rich features lead to an average gain of $1.3\%$ and $3.1\%$ over basic features using balanced scaffold split and scaffold split, respectively. Specifically, it achieves $76.7\%$ vs $78.0\%$ for balanced scaffold split, and $68.7\%$ vs $71.8\%$ on scaffold split. The gain brought by the rich features are more significant than the ones with different self-supervised pretraining objectives. \tabref{tab:Balanced scaffold + basic feature + unsupervised} to \tabref{tab:Scaffold + basic feature +  supervised} show that pretraining has more positive impact when basic features are used. In particular, the self-pretraining with context prediction shows significant gains especially in the {scaffold split} setting. However, the gain diminishes when careful feature engineering are applied to the downstream tasks (use rich feature in \emph{vanilla configuration}). The supervised pretraining continues the significant gain under these settings, which shows the consistency and reliability of the situation with the labeled and downstream-task-aligned supervisions. %Specifically, the gain brought by supervised pretraining can be more significant than the rich feature engineering alone. 
%\vspace{-7.5mm}
\subsection{Pretraining datasets}
\label{sec:exp_data_size}
%\vspace{-2mm}
\begin{table*}[t]
\centering
%\vspace{-5mm}
\caption{\textbf{Large scale pretraining data} with balanced scaffold split. No pretraining gets an average AUC of 78.0\%. \label{tab:savi-balanced-split}}
\vspace{2mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllr}
%\hline
\Xhline{2\arrayrulewidth}
Methods        & \textbf{BBBP}  & \textbf{BACE}  & \textbf{TOX21} & \textbf{TOXCAST} & \textbf{SIDER}   & \textbf{AVE GAIN}\\ 
%\hline
\Xhline{2\arrayrulewidth}
\nopretrain      & 92.23($\pm$3.07) & 87.43($\pm$1.63)     & 79.2($\pm$1.99)  & 69.13($\pm$0.55) & 61.92($\pm$0.89) & 0($\pm$1.626)\\
\masktask     & 92.33($\pm$2.08) & 87.22($\pm$1.79) & 79.12($\pm$1.62) & 69.47($\pm$0.65)   & 61.24($\pm$1.94)  &  -0.106($\pm$1.616)  \\
\contexttask  &  93.32($\pm$0.53) & 87.77($\pm$2.94) & 79.18($\pm$2.48) & 70.13($\pm$0.56) & 62.24($\pm$2.65)  &  0.546($\pm$1.832) \\ 
\Xhline{2\arrayrulewidth}
\rowcolor{Gray}
\supervisedmasktask     & 93.23($\pm$3.02) & 86.39($\pm$1.67) & 81.89($\pm$1.58) & 71.77($\pm$0.50)  & 63.73($\pm$2.20)   &  1.420($\pm$1.794) \\
\rowcolor{Gray}
\supervisedcontexttask & 92.55($\pm$2.93) & 87.76($\pm$1.87) & 82.19($\pm$1.58) & 72.91($\pm$0.71) & 62.44($\pm$0.45)  &  1.588($\pm$1.508) \\
%\hline
\Xhline{2\arrayrulewidth}
 %\vspace{-10mm}
\end{tabular}%
}
\end{table*}


\begin{table*}[t]
% \small
\caption{\textbf{Large scale pretraining} data with scaffold split. No pretraining gets an average AUC of 71.8\%. \label{tab:SAVI-scaffold-split}}
%\vspace{-3mm}
\vspace{2mm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllr}
%\hline
\Xhline{2\arrayrulewidth}
Methods               & \textbf{BBBP}  & \textbf{BACE} & \textbf{TOX21} & \textbf{TOXCAST} & \textbf{SIDER}  &  \textbf{AVE GAIN}\\ 
%\hline
\Xhline{2\arrayrulewidth}
\nopretrain             & 74.83($\pm$0.73) & 80.10($\pm$0.42) & 75.86($\pm$0.58)  & 65.95($\pm$0.15) & 62.30($\pm$1.14)  & 0($\pm$0.604)\\
\masktask               & 73.81($\pm$1.82) & 81.90($\pm$1.59) & 74.94($\pm$0.05) & 66.95($\pm$0.12)  & 62.93($\pm$0.34)  &  0.298($\pm$0.784) \\
\contexttask            & 74.32($\pm$0.85) & 83.93($\pm$0.24) & 74.42($\pm$0.19) & 67.01($\pm$0.29)  & 64.83($\pm$0.45)  & 1.094($\pm$0.404)\\ 
\Xhline{2\arrayrulewidth}
\rowcolor{Gray}
\supervisedmasktask     & 73.32($\pm$0.60) & 83.38($\pm$1.05) & 78.59($\pm$0.09) & 67.01($\pm$0.18)  & 65.40($\pm$0.12)  & 1.732($\pm$0.408)\\
\rowcolor{Gray}
\supervisedcontexttask  & 74.38($\pm$0.93) & 86.33($\pm$0.16) & 78.16($\pm$0.25) & 68.71($\pm$0.07)  & 62.22($\pm$0.48)  & 2.152($\pm$0.378)\\
%\hline
\Xhline{2\arrayrulewidth}
%\vspace{-10mm}
\end{tabular}%
}
\end{table*}

As observed in natural language processing domain, more text pretraining data lead to better downstream performance. Intuitively this can be true for molecule representation domain as well, so we run a new set of experiments with the model pretrained on SAVI dataset, which is about 500 times larger than the ZINC15 dataset we used in the above result sections. We present the results pretrained on SAVI dataset using balanced scaffold split or scaffold split in \tabref{tab:savi-balanced-split} and \tabref{tab:SAVI-scaffold-split}, respectively. Other configurations are the same as the \emph{vanilla configuration}. 

Compared with the performance on ZINC15, the SAVI pretraining data does not lead to a significant improvement either on balanced scaffold split  (\tabref{tab:unsupervised-obj} vs \tabref{tab:savi-balanced-split}) or scaffold split (\tabref{tab:split} or \tabref{tab:SAVI-scaffold-split}). Similarly, the self-supervised pretraining objectives lead to negligible gain on downstream task performance, while the supervised one still achieves a clear gain. 

As the result is counterintuitive, we further investigate the reason behind it by inspecting the pretraining performances with different training objectives on both ZINC15 and SAVI datasets. We plot the curve of accuracy growth with the number of training steps iterated. We can see from \Figref{fig:pretraining} that in all settings the pretraining accuracy grows above 90\% quickly after only 0.1 to 0.2M steps and also converges quickly. Given that the model gets very high accuracy without even going through 1 epoch of the SAVI dataset, it is expected that the larger training data like SAVI may not provide more learning signals for the model, and partially explains why more molecules wouldn't help significantly in this case. Furthermore, these figures might suggest several reasons of why the self-supervised pretraining may not be very effective in some situations:
\begin{itemize}[noitemsep,topsep=2pt,parsep=6pt,partopsep=2pt, leftmargin=*]
	\item \textbf{Tasks are easy.} Some of the self-pretraining tasks for molecules might be easy, so that model learns less useful information from pretraining. For example in the masked node prediction case, the model is expected to predict the atomic number from a vocabulary with less than 100 candidate atoms. Furthermore, due to the valence constraints, the graph topology may already exclude most of the wrong atoms. As a comparison, the vocabulary size for text pretraining may be 100k or even higher. Some structured prediction tasks like context prediction might be hard, but due to the difficulty of structured prediction itself and the proposal for high quality negative examples for contrastive learning, it can still be challenging for downstream task improvements. Other strategies like motif prediction can be achieved by subgraph matching, which can be easy for GNN that intrinsically does the graph isomorphism test.
	\item \textbf{Data lacks diversity.} Due to biophysical and functional requirements, molecules share many common sub-structures, e.g., functional motifs. Hence, molecules may not be as diversified as text data. This is why the model learns to generalize quickly within the training distribution. 
	\item \textbf{2D Structure is not enough to infer functionality.} Some important biophysical properties (such as 3D structure, chirality) are barely reflected in the 2D-feature-based pretraining (e.g., using smiles or 2D graph features). For example, the molecules with the same chemical formula and 2D feature, can have very different chirality, which leads to quite different toxicity \citep{smith2009chiral} (e.g. flipped toxicity labels). This is not captured in the current GNN pretraining frameworks that we considered.
\end{itemize}
%\vspace{-1mm}


%\begin{wrapfigure}{r}{0.5\textwidth}
%\begin{figure}%[t]
%\centering
%\includegraphics[width=0.46\textwidth]{figs/pretrain-4.pdf}
%\caption{Pretraining accuracy on ZINC15 or SAVI datasets with node prediction or context prediction objectives. \label{fig:pretraining}}
%\vspace{-1mm}
%\end{figure}
%\end{wrapfigure}


\begin{wrapfigure}{r}{0.59\textwidth}
 \vspace{-9mm}
  \begin{center}
    \includegraphics[width=0.36\textwidth]{figs/pretrain-4.pdf}
  \end{center}
  \vspace{-3mm}
 \caption{Pretraining accuracy on ZINC15 or SAVI datasets with node prediction or context prediction objectives. \label{fig:pretraining}}
 \vspace{-3mm}
\end{wrapfigure}
%\subsection{GNN architecture} 
%We also investigate GNN
% \vspace{-4mm}
\subsection{Hyper-parameters for downstream tasks}
We also find that hyper-parameters for downstream tasks are critical for the their performance that their choices may change the conclusion of the effectiveness of pretraining in some settings.
% For example, learning rate is important. 
We can take the learning rate as an example.
As the models initialized from scratch and pretraining may have different scales, the most suitable learning rate required for downstream tasks may also be different. Without tuning learning rate extensively, we may reach a misleading conclusion.
In particular, when we adopt the default learning rate for reproducing the existing success of pretraining in \tabref{tab:feature-balancedscaffold-basicfeature-wrong} of Appendix~\ref{sec:reproduce}, we indeed observe the advantage of pretraining. However, if we follow our procedures (e.g. extensive search learning rate and averaging over three splits), the resulting \tabref{tab:unsupervised-obj} and \tabref{tab:super-obj} indicate no performance gain by pretraining. So we suggest that the evaluation of pretraining should consider the hyper-parameter tuning and averaging over different splits. 







==> [NeurIPS2022] Graph pretraining/summary.tex <==
%\vspace{-1mm}
\section{Summary and takeaways}
\label{sec:summary}
%\vspace{-1mm}
Based on our experiments in \secref{sec:results}, we present our takeaways by empirically summarizing our conjectures on when the pretraining would/would not help the molecular representation learning.
%\vspace{-3mm}
\paragraph{When pretraining might help} We find it typically helps 1) if we can have the supervised pretraining with target labels that are aligned with the downstream tasks. However, getting large amount of high-quality and relevant supervision is not always feasible; 2) if the high quality hand-crafted features are absent. However, it seems that the gain obtained by self-supervised pretraining is not as significant as these high quality hand-crafted features based on our current studies; 3) if the downstream train, valid and test dataset distributions are substantially different.
%\vspace{-3mm}
\paragraph{When the gain diminishes?} In some situations the gain of pretraining might diminish 1) if we already have the high quality hand-crafted features (e.g. rich features described in \secref{sec:design_choice}); 2) if we don't have the highly relevant supervisions. As shown in \secref{sec:exp_data_size}, many self-supervised pretraining tasks might be too easy for the model to learn meaningful embedding; 3) if the downstream data splits are balanced; 4) if the self-supervised learning dataset lacks diversity, despite its scale.
\paragraph{Why pretraining may not help in some cases?} In our paper we pretrained a GNN on a much larger dataset (SAVI) than before, hoping to replicate gain of pretraining like in NLP domain. However, we do not obtain the expected gain. The pretraining accuracy curve (\Figref{fig:pretraining}) provides some potential explanations of why pretraining may not work: some of the pretraining accuracy curve grows above $95\%$+ quickly and converges fast, unlike pretraining in NLP which keeps growing to $70\%$ and hardly plateaus. This suggests that some of the pretraining methods like masked node label prediction might be easy (as the vocabulary size is much smaller compared to NLP) and therefore transfer less knowledge for downstream tasks.


==> [NeurIPS2022] Graph pretraining/summary_table.tex <==
\begin{table*}[th]
\centering
%\vspace{-5mm}
\caption{Summary of Experiments. \tabref{tab:graphsage + neurips split} and \tabref{tab:graphsage + iclr split} are deferred to appendix due to space limit. \label{tab:summary-table}}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{c|cc|cc|cc|cc|cc}
%\hline
\Xhline{2\arrayrulewidth}
 &
  \multicolumn{2}{c|}{\textbf{Pretrain Objective}} &
  \multicolumn{2}{c|}{\textbf{Graph Features}} &
  \multicolumn{2}{c|}{\textbf{Downstream Splits}} &
  \multicolumn{2}{c|}{\textbf{GNN Arch}} &
  \multicolumn{2}{c}{\textbf{Pretrain Dataset}} \\ 
  \cline{2-11}
  %\xchline{2-11}{2\arrayrulewidth}
 &
{Self-Supervised} &
{Supervised} &
{Rich} &
{Basic} &
{Balanced} &
{Scaffold} &
{GIN} &
{GraphSage} &
{ZINC15} &
{SAVI} \\
  %\hline
  \Xhline{2\arrayrulewidth}
\textbf{\tabref{tab:unsupervised-obj}} 
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:super-obj}} 
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:split}} 
   &\ding{52}
   &
   &\ding{52}
   &
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:feature-scaffold-richfeature-supervised}} 
   &
   &\ding{52}
   &\ding{52}
   &
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:Balanced scaffold + basic feature + unsupervised}} 
   &\ding{52}
   &
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:Balanced scaffold + basic feature + supervised}}
   &
   &\ding{52}
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:Scaffold + basic feature + unsupervised} }
   &\ding{52}
   &
   &
   &\ding{52}
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
\textbf{\tabref{tab:Scaffold + basic feature + supervised}}
   &
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   \\\hdashline
%\textbf{\tabref{tab:graphsage + neurips split}} 
%   &\ding{52}
%   &\ding{52}
%   &\ding{52}
%   &
%   &\ding{52}
%   &
%   &
%   &\ding{52}
%   &\ding{52}
%   &
%   \\ \hdashline
%\textbf{\tabref{tab:graphsage + iclr split}} 
%   &\ding{52}
%   &\ding{52}
%   &\ding{52}
%   &
%   &
%   &\ding{52}
%   &
%   &\ding{52}
%   &\ding{52}
%   &
%   \\\hdashline
\textbf{\tabref{tab:savi-balanced-split}} 
   &\ding{52}
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   &\ding{52}
   & 
   &
   &\ding{52}
   \\\hdashline
\textbf{\tabref{tab:SAVI-scaffold-split}} 
   &\ding{52}
   &\ding{52}
   &\ding{52}
   &
   &
   &\ding{52}
   &\ding{52}
   &
   &
   &\ding{52}
   \\ 
   %\hline
  % \Xhline{2\arrayrulewidth}
  \hdashline 
   \textbf{\tabref{tab:graphsage + neurips split}} 
   &\ding{52}
   &\ding{52}
   &\ding{52}
   &
   &\ding{52}
   &
   &
   &\ding{52}
   &\ding{52}
   &
   \\ \hdashline
\textbf{\tabref{tab:graphsage + iclr split}} 
   &\ding{52}
   &\ding{52}
   &\ding{52}
   &
   &
   &\ding{52}
   &
   &\ding{52}
   &\ding{52}
   &
   \\\hdashline
     \Xhline{2\arrayrulewidth}
\end{tabular}%
%\vspace{-5mm}
}
\end{table*}


